$\epsilon$-net Induced Lazy Witness Complexes on Graphs

Computation of persistent homology of simplicial representations such as the Rips and the C\v{e}ch complexes do not efficiently scale to large point clouds. It is, therefore, meaningful to devise approximate representations and evaluate the trade-off between their efficiency and effectiveness. The lazy witness complex economically defines such a representation using only a few selected points, called landmarks. Topological data analysis traditionally considers a point cloud in a Euclidean space. In many situations, however, data is available in the form of a weighted graph. A graph along with the geodesic distance defines a metric space. This metric space of a graph is amenable to topological data analysis. We discuss the computation of persistent homologies on a weighted graph. We present a lazy witness complex approach leveraging the notion of $\epsilon$-net that we adapt to weighted graphs and their geodesic distance to select landmarks. We show that the value of the $\epsilon$ parameter of the $\epsilon$-net provides control on the trade-off between choice and number of landmarks and the quality of the approximate simplicial representation. We present three algorithms for constructing an $\epsilon$-net of a graph. We comparatively and empirically evaluate the efficiency and effectiveness of the choice of landmarks that they induce for the topological data analysis of different real-world graphs.

==> ATDA2019(cr)/Algos.tex <==
\section{Algorithms for Computing $\epsilon$-Net}\label{sec:algos}
In this section, we propose and elaborate three algorithms, namely Greedy-$\epsilon$-Net, Iterative-$\epsilon$-Net, and SPTprunning-$\epsilon$-net, for computing $\epsilon$-net on graphs. 
\vspace{-1em}
\subsection{Greedy-$\epsilon$-Net Algorithm}\vspace{-1em}
We propose a greedy algorithm, namely Greedy-$\epsilon$-Net, to compute a minimal-cardinality $\epsilon$-net of a graph. Greedy-$\epsilon$-Net (\Cref{alg:base}) maintains a hash table with vertices as keys and the number of vertices in their $\epsilon$-cover as values. At each step, Greedy-$\epsilon$-Net selects a vertex with the largest $\epsilon$-cover, marks the covered vertices, and updates the $\epsilon$-cover of other vertices until all the vertices are marked as covered.

% \textbf{Time-complexity.}
% Let $n$ be the number of vertices and $m$ be the number of edges of a graph. The complexity of the algorithm $\epsilon$-BFS is $O(n^3)$, since it runs BFS for each vertex. Line 7 - 22 runs in $O(|K|(n\log{n} + n^2))$ time, where $K = (\frac{\Delta}{\epsilon})^{O(\log(\frac{|V|}{\epsilon}))}$.
% Thus, Greedy-$\epsilon$-net has a time-complexity of $O(n^3)$.
\vspace{-1em}
\subsection{Iterative-$\epsilon$-Net Algorithm}\vspace{-1em}
Iterative-$\epsilon$-Net (\Cref{alg:idif}) is a diffusive algorithm that maintains a set $C_{(\epsilon,2\epsilon)}$ that contains the set of unmarked vertices that are within a ring of $(\epsilon,2\epsilon]$ distance from the current set of landmarks. We call them the \textbf{ring vertices}.
Iterative-$\epsilon$-Net also maintains another set $C_{2\epsilon}$ that contains the set of unmarked vertices that are at distance at least $2\epsilon$ but are adjacent to the bordering vertices of the cover. We call them the \textbf{enveloping vertices}.

Iterative-$\epsilon$-net, at each iteration, uniformly at random selects a vertex $u$ from the current set of enveloping vertices as next landmark, and run Partial-BFS (\Cref{alg:pbfs}) starting at $u$ to mark the vertices in its $\epsilon$-cover, as well as to update the enveloping and ring vertex sets. If enveloping vertex set is empty it selects a ring vertex uniformly at random as next landmark.

Iterative $\epsilon$-net algorithm has the property that some vertex in the $\epsilon$-cover of landmark $l_{i+1}$ is always adjacent to some vertex in the $\epsilon$-cover of landmark $l_i$. Thus the two covers are adjacent as sets.\vspace*{-1pt}

% \textbf{Time-complexity.}
% The run-time of algorithm Iterative-$\epsilon$-net is $O(n+m)$ since Algorithm~\ref{alg:pbfs} marks every vertex irrespective of the value of $\epsilon$ and the number of landmarks chosen by Iterative-$\epsilon$-net algorithm. 

\begin{algorithm}[t!]
\caption{Iterative-$\epsilon$-Net}
\label{alg:idif}
\begin{algorithmic}[1]
% {\color{blue}
\Require Graph $G = (V,E,W)$, parameter $\epsilon$
\Ensure Set of landmarks $L$
\State Initialise $L = \phi$
\State $i = 1$
% \STATE Let $j$ be a random integer from $[1,\cdots,n]$
% \STATE Initial landmark $l_1 = p[j]$
% \STATE Initialize candidate points $C[1 \cdots n] = P$
\State Select initial landmark $l_i= u$ uniformly at random from $V$.
\State $L = L \cup \{u\}$
\State Let $C^{u}_{(\epsilon,2\epsilon)}$  be the set of unmarked vertices $v$ such that $\epsilon < d_G(u,v) \leq 2\epsilon$.
\State Let $C^{u}_{2\epsilon}$ be the set of vertices $v$ such that $d_G(u,v)>2\epsilon$ and are the closest.
 \Repeat 
    \State $C^{u}_{\epsilon,2\epsilon} = \textbf{PartialBFS}(G,l_i,C^{u}_{(\epsilon,2\epsilon)},C^{u}_{2\epsilon})$ 
    \If{$C^{u}_{2\epsilon}$ is empty}
        \State select $l_{i+1}$ uniformly at random from $C^{u}_{(\epsilon,2\epsilon)}$.
    \Else
        \State select $l_{i+1}$ uniformly at random from $C^u_{2\epsilon}$.
    \EndIf
    % \State Find the first $\delta =   [1,2,\cdots,\log(\ceil{\Delta/2\epsilon})]$ for which $N^i_{(2^\delta\epsilon,2^{\delta+1}\epsilon)}$ contains some unmarked points.
    % \State Set $C_i = C_i \cup  N^i_{(2^\delta\epsilon,2^{\delta+1}\epsilon)}$
    % \EndIf
    % \State Select $l_{i+1}$ u.a.r from $C^{u}_{(\epsilon,2\epsilon)}$.
    \State $L = L \cup \{l_{i+1}\}$.
    \State $i = i + 1$
    \State $u = l_{i+1}$
 \Until{all vertices are marked}
% }
\end{algorithmic}
\end{algorithm}
\begin{algorithm}[t!]
\caption{PartialBFS}
\label{alg:pbfs}
\begin{algorithmic}[1]
\Require Graph $G$, vertex $u$, set $C^{u}_{(\epsilon,2\epsilon)}$, set $C^{u}_{2\epsilon}$.
% \Ensure Set of Candidate landmarks $C^u$
\State Initialise Queue $Q = \{u\}$
\State $u.marked$ = True

 \While{$Q \neq \phi$} 
    \State $v = \text{DEQUEUE}(Q)$
    \ForAll{ $v' \in G.Adj[v]$}
    \If{ $v'.marked$ = False}
        \State $v'.d = v.d + W[v,v']$
        \If{ $v'.d \leq \epsilon$}
            \State $v'.marked$ = True
            \State Remove $v'$ from $C^{u}_{(\epsilon,2\epsilon)}$ and $C^{u}_{2\epsilon}$ if exists.
            \State $\text{ENQUEUE}(Q,v')$
        \ElsIf{$\epsilon< v'.d \leq 2\epsilon$}
            \State $C^{u}_{(\epsilon,2\epsilon)} = C^{u}_{(\epsilon,2\epsilon)} \cup \{v'\}$
            \State $\text{ENQUEUE}(Q,v')$
        \Else
            \State $C^{u}_{2\epsilon} = C^{u}_{2\epsilon} \cup \{v'\}$
        \EndIf
    \EndIf
    
    \EndFor
 \EndWhile
% }
\end{algorithmic}
\end{algorithm}
%% End of Baseline
\vspace*{-.5em}
\subsection{Sparsity based Pruning Algorithm on Shortest Path Tree}\vspace*{-.5em}
%{\color{red}We propose algorithm~\ref{alg:treeeps} that constructs a shortest path tree of the graph to select landmarks prune a few landmarks to construct $\epsilon$-net of the graph. }
We propose SPTpruning-$\epsilon$-Net algorithm (Algorithm~\ref{alg:treeeps}) that constructs a shortest path tree of the graph and uses the tree to compute an $\epsilon$-net.
Algorithm~\ref{alg:treeeps} computes a shortest path tree rooted at a vertex chosen uniformly at random. The algorithm uses $\epsilon$-BFS (Algorithm~\ref{alg:ebfs}) to construct a preliminary BFS spanning tree of the graph (line 2). Then the algorithm constructs an $\epsilon$-net of the BFS-tree (line 4-28). It does so by traversing the tree level-order starting from root, running $\epsilon$-BFS in the tree to mark covered vertices, and add the set of unmarked vertices at level $\epsilon+1$  as candidates for landmarks. 

An $\epsilon$-net $L_{SPT}$ of a BFS-tree $SPT(G)$ of a graph $G$ has the property that, any vertex $v \in SPT(G) \subset G$ that is covered by some vertex $u \in L_{SPT}$, is also covered by the $u \in V$ in the graph as well. This property follows from the fact that, the distance between any vertex pair $d_G(u,v)$ in the graph can only be shorter than their distance $d_{SPT}(u,v)$ in the BFS-tree. 

Unless one of the vertex is a root, the distance between any pair of vertices in the tree is not guaranteed to be the shortest in the graph. Thus an $\epsilon$-net of a BFS-tree does not have $\epsilon$-sparsity in the graph containing the BFS-tree as a subgraph. As a remedy, Algorithm~\ref{alg:prune} prunes vertices from the candidate landmarks that are covered by other candidate landmark. 

% \textbf{Time-complexity.}
% Line 2 has complexity $\Theta(n+m)$. Size of Shortest path tree SPT is $\Theta(n)$. Line 7-27 runs in $\Theta(n)$ time, since it is a BFS on the Shortest Path tree. Pruning algorithm in algorithm~\ref{alg:prune} runs in $O(n+m)$ time, since it has to traverse every vertex and edge in the worst case (when $\epsilon=0$) to 

\begin{algorithm}[t!]
\caption{SPTpruning-$\epsilon$-net}
\label{alg:treeeps}
\begin{algorithmic}[1]
\Require Graph $G$, Diameter $\Delta$, parameter $\epsilon$
\Ensure Set of landmarks $C$
\State Select a vertex $u$ uniformly at random from $V$.
\State Run \textbf{$\epsilon$-BFS(G,u,$\Delta$)} to construct a BFS spanning tree rooted at $u$
\State Let $SPT$ be the tree.
\State Initialise Queue $Q = \{u\}$
\State $u.marked$ = True
\State Let $\epsilon$-net of the SPT $C_\epsilon = \phi$ 
\Repeat 
 \While{$Q \neq \phi$} 
    \State $u' = \text{DEQUEUE}(Q)$
    \State u'.marked = True
    \State $u'.d = 0$
    \State Initialise Queue $Q' = \{u'\}$
    \While{$Q' \neq \phi$} 
        \State $v = \text{DEQUEUE}(Q')$
        \ForAll{ $v' \in SPT.Adj[v]$}
        \If{ $v'.marked$ = False}
            \State $v'.d = v.d + W[v,v']$
            \If{ $v'.d \leq \epsilon$}
                \State $v'.marked$ = True
                \State $\text{ENQUEUE}(Q',v')$
            \Else
                \State $C_\epsilon = C_{\epsilon} \cup \{v'\}$
                \State $\text{ENQUEUE}(Q,v')$
            \EndIf
        \EndIf
        
        \EndFor
    \EndWhile
 \EndWhile
 \Until{All vertex in $SPT$ are marked}
\State C = Prune(G,$C_\epsilon$,$\epsilon$)
\end{algorithmic}
\end{algorithm}
\begin{algorithm}[t!]
\caption{Prune}
\label{alg:prune}
\begin{algorithmic}[1]
\Require Graph $G$, A set of landmarks $C_\epsilon$, parameter $\epsilon$
\Ensure Set of landmarks $C$
\State $C = C_\epsilon$
\ForAll{vertex $v \in C_\epsilon$}
    \If {v.marked = False}
        \State Run \textbf{$\epsilon$-BFS(G,v,$\epsilon$)}
    \Else
        \State $C = C \setminus \{v\}$
    \EndIf
\EndFor
\end{algorithmic}
\end{algorithm}


% \subsection{Reverse Diffusive algorithm}
% ~\Cref{alg:kr} is a modification of kruskal's algorithm for finding a minimum spanning tree. 

% {\color{blue}{The algorithm starts with all vertices in the graph as unmarked. Then the algorithm processes edges in ascending order of edge weights. At each iteration, it adds the unmarked endpoint of an edge to the $\epsilon$-covers of the marked endpoint and mark it when the distance from the unmarked vertex to the root of the tree containing the marked endpoint is at most $\epsilon$. 

% If both endpoints of an edge is unmarked the algorithm selects one of the arbitrarily chosen endpoint as root. The algorithm stops when all the vertices are marked as covered. In the end, all the roots of the trees in the forest are reported as landmarks.}}

% \begin{algorithm}[!htbp]
% \caption{ Kruskal$\epsilon$-net}
% \label{alg:kr}
% \begin{algorithmic}[1]
% % {\color{blue}
% \Require Graph $G = (V,E,W)$, parameter $\epsilon$
% \Ensure Set of Landmarks $L$
% \State Initialise $L = \phi$
% % \State Let $nc$ be the hash table of $\epsilon$-cover size of the vertices in $V$.
% \ForAll{$u \in V$}
%     \State MAKE-SET($u$)
%     \State $d[u] = 0$
%     \State $marked[u]$ = False
% \EndFor
% % \State Sort $nc$ in descending order of its value. 
% % \State Initialize hash table $marked[]$ to False for each $u \in V$
% \State Sort $E$ in ascending order of $W$
% \ForAll{$(u, v) \in E$ till there are unmarked vertices:}
%     \If {FIND-SET($u$) $\neq$ FIND-SET($v$)}
%         \If {$marked[u] = True$ \& $marked[v] = True$}
%             % \Comment{Cross Edge between two covers}
%             \State Do nothing
%         \ElsIf {$marked[u] = False$ \& $marked[v] = True$}
%             \If{$d[v] + W[u,v] \leq \epsilon$} 
%                 \State $d[u] = d[v] + W[u,v]$
%                 \State UNION($u$,$v$)
%                 \State Mark $u$
%             \EndIf 
%         \ElsIf {$marked[v] = False$ \& $marked[u] = True$}
%             \If{$d[u] + W[u,v] \leq \epsilon$} 
%                 \State $d[v] = d[u] + W[u,v]$
%                 \State UNION($u$,$v$)
%                 \State Mark $v$
%             \EndIf 
%         \Else 
%             \If {$w[u,v] \leq \epsilon$ }
%                 \State UNION($u$,$v$)
%                 \If{FIND-SET($u$) == v}
%                     \State $d[u] = W[u,v]$ 
%                 \Else 
%                     \State $d[v] = W[u,v]$
%                 \EndIf                
%                 \State Mark $u$ and $v$
%             \EndIf
%         \EndIf
%     \EndIf
% \EndFor
% \State L = List of vertices $u$ for which FIND-SET($u$) $== u$.
% \end{algorithmic}
% \end{algorithm}

==> ATDA2019(cr)/README <==
This package provides a class for typesetting publications of 
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see
Installation section of the User's Guide.

Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.  
		Footnotes rearranged.
                Option natbib is now mostly superfluous: the class 
		makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
		Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
		file is used for all styles.  Better treatment
		of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend;  should be 
		invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29	Documentation changes.  Head height increased from 12pt to 13pt.
		Removed spurious indent at start of abstract.
		Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
	        Added \frenchspacing.
		\department now has an optional hierarchy level.
		Switched to T1 encoding
		Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
		(thanks to Matteo Riondato)
		Table of contents now works
		Marginalia now work in all formats
		New command \additionalaffiliation
		Documentation changes

version 1.32    New DOI formatting.
		Format siggraph is now obsolete, and sigconf
		is used instead.
		New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
		New option `authordraft'
                Documentation updates
		Bug fixes
		We now use Type 1 versions of Libertine fonts even with XeTeX.
		New hook acmart-preload-hook.tex (wizards only!)
		Added new options `obeypunctuation' for \affiliation command
		Added SubmissionID
		Added right line count ruler for two-column formats
		Added workaround for Adobe Acrobat bugs in selection
		Added eid field to the bibliography
		
version 1.34    Deleted DOI from doi numbers
		Changed bibstrip formatting
		The command \terms is now obsolete
		The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.


==> ATDA2019(cr)/algo_1.tex <==
%% Baseline
\setlength{\textfloatsep}{6pt}% Remove \textfloatsep
\begin{algorithm}[t!]
\caption{Greedy-$\epsilon$-Net}
\label{alg:base}
\begin{algorithmic}[1]
% {\color{blue}
\Require Graph $G = (V,E,W)$, parameter $\epsilon$
\Ensure Set of Landmarks $L$
\State Initialize $L = \phi$
\State Let $nc$ be the hash table with vertices as keys, number of vertices in their $\epsilon$-cover as value.
\ForAll{$u \in V$}
    \State $nc[u] =$ \textbf{$\epsilon$-BFS$(G,u,\epsilon)$}
\EndFor
\State Initialize all vertex $u \in V$ as marked.
\Repeat
    \State Sort $nc$ in descending order of its value. 
    \If{ $marked[u]$ = False}
        \State $L.insert(u)$
        \ForAll{vertex $u'$ in u's $\epsilon$-cover}
            \State Mark $u'$ as True.
            \State Delete key $u'$ from nc.
            \ForAll{$v \in V$}
                \If{$u'$ is in $\epsilon$-cover of $v$}
                    \State Decrease $nc[v]$ by 1.
                \EndIf
            \EndFor
        \EndFor
    \EndIf
    \State Delete key $u$ from nc.
\Until{all vertices are marked} 
% \State Let $C^{u}_{(\epsilon,2\epsilon)}$  be the set of unmarked vertices that are at least $\epsilon$ and at most $2\epsilon$ geodesic distance from vertex $u$.
%  \Repeat 
%     % \State Let, $N^i_{\leq\epsilon}$ be the set of points at distance less than $\epsilon$ from $l_i$.
%     % \State Mark all points in $N^i_{\leq\epsilon}$ as covered.
%     % \STATE Let $N^i_{(\epsilon,2\epsilon)}$ be the set of points at distance less than $2\epsilon$ and greater than $\epsilon$ from $l_i$.
%     \State $C^{u}_{\epsilon,2\epsilon} = \textbf{PartialBFS}(G,l_i,\epsilon)$ 
%     \If{$C^{u}_{(\epsilon,2\epsilon)}$ is empty}
%     \State $\delta = 1$
%     \Repeat
%         \State $C^{u}_{(\epsilon,2\epsilon)} = \textbf{PartialBFS}(G,l_i,2^\delta)$ 
%         \State $\delta = \delta + 1$
%      \Until{all vertices are marked or $C^{u}_{(\epsilon,2\epsilon)} \neq \phi$}
%     % \State Find the first $\delta =   [1,2,\cdots,\log(\ceil{\Delta/2\epsilon})]$ for which $N^i_{(2^\delta\epsilon,2^{\delta+1}\epsilon)}$ contains some unmarked points.
%     % \State Set $C_i = C_i \cup  N^i_{(2^\delta\epsilon,2^{\delta+1}\epsilon)}$
%     \EndIf
%     \State Select $l_{i+1}$ u.a.r from $C^{u}_{(\epsilon,2\epsilon)}$.
%     \State $L = L \cup \{l_{i+1}\}$.
%     \State i = i + 1
%  \Until{all vertices are marked}
% }
\end{algorithmic}
\end{algorithm}
\begin{algorithm}[t!]
\caption{$\epsilon$-BFS}
\label{alg:ebfs}
\begin{algorithmic}[1]
\Require Graph $G = (V,E,W)$, vertex $u$, parameter $\epsilon$.
\Ensure Set of vertices in $u$'s $\epsilon$-cover, $C_\epsilon$
\State Initialize Queue $Q = \{u\}$
\State initialize $C_\epsilon = \phi$
 \While{$Q \neq \phi$} 
    \State $v = \text{DEQUEUE}(Q)$
    \State $v.marked$ = True
    \ForAll{ $v' \in G.Adj[v]$}
        \If{ $v'.marked$ = False}
            \State $v'.d = v.d + W[v,v']$
            \If{ $v'.d \leq \epsilon$}
                \State $C_\epsilon = C_\epsilon \cup \{v'\}$
            \EndIf
        \EndIf
    \EndFor
 \EndWhile
% }
\end{algorithmic}
\end{algorithm}



==> ATDA2019(cr)/algorithms.tex <==
% \section{Construction of $\epsilon$-nets from graphs}
% \label{sec:construction_graph}

% \subsection{$\epsilon$-net construction for graphs}
% We propose the following algorithm \textbf{Baseline$_\epsilon$} to compute $\epsilon$-net of a graph as the baseline construction. 

\input{Algos.tex}
% Kruskal-style

% \begin{algorithm}[t!]
% \caption{ Kruskal$\epsilon$-net}
% \label{alg:1}
% \begin{algorithmic}[1]
% % {\color{blue}
% \Require Graph $G = (V,E,W)$, parameter $\epsilon$
% \Ensure Set of Landmarks $L$
% \State Initialize $L = \phi$
% % \State Let $nc$ be the hash table of $\epsilon$-cover size of the vertices in $V$.
% \ForAll{$u \in V$}
%     \State $C_u = \{u\}$
%     \State $d.u = 0$
% \EndFor
% % \State Sort $nc$ in descending order of its value. 
% \State Initialize hash table $marked[]$ to False for each $u \in V$
% \ForAll{$(u, v)$ in $E$ ordered by $w[u,v]$, increasing:}
%     \If {All vertices marked}
%         \State Break
%     \EndIf
%     \If {FIND-SET(u) $\neq$ FIND-SET(v)}
%         \If {$marked[u] = True$ \& $marked[v] = True$}
%             % \Comment{Cross Edge between two covers}
%             \State Do nothing
%         \ElsIf {$marked[u] = False$ \& $marked[v] = True$}
%             \If{$d.v + w[u,v] \leq \epsilon$} 
%                 \State $C_{\text{FIND-SET}(v)} = C_{\text{FIND-SET}(v)} \cup \{u\}$
%                 \State $d.u = d.v + w[u,v]$
%                 \State Mark $u$
%             \EndIf 
%         \ElsIf {$marked[v] = False$ \& $marked[u] = True$}
%             \If{$d.u + w[u,v] \leq \epsilon$} 
%                 \State $C_{\text{FIND-SET}(u)} = C_{\text{FIND-SET}(u)} \cup \{v\}$
%                 \State $d.v = d.u + w[u,v]$
%                 \State Mark $v$
%             \EndIf 
%         \Else 
%             \If {$w[u,v] \leq \epsilon$ }
%                 \State $d.v = d.v + w[u,v]$ // Assuming $u<v$
%                 \State $C_u$ =UNION($C_u$,$C_v$)
%                 \State Mark $u$ and $v$
%             \EndIf
%         \EndIf
%     \EndIf
% \EndFor
% \State L = All the set representatives
% % \ForAll{$u$ = nc.Keys()}
% %     \If{ $marked[u]$ == False}
% %         \State $L.insert(u)$
% %         \State Mark all the vertices in $u$'s $\epsilon$-cover as False.
% %     \EndIf
% % \EndFor 
% \end{algorithmic}
% \end{algorithm}

%% End kruskal style




% {\color{red}{\textbf{Proof of correctness. Need to revisit this correctness in light of the definitions}

% For any vertex $v \in V$, the length of the shortest path from $v$ to the landmark $l$ nearest from $v$ in tree $T_m$ is at most $\epsilon$. Since a shortest path in $G$ is the smallest among all paths, the length of the shortest path from $v$ to $l$ is graph $G$ is at most $\epsilon$. 
% }}

% In the subsequent sections we use `$\epsilon$-net landmarks' to imply `an $\epsilon$-net that induces a lazy witness filtration irrespective of its construction'. 
%In the subsequent sections, We use `$\epsilon$-net-rand landmarks' to imply landmarks constructed by the $\epsilon$-net-rand algorithm, and so on for the other algorithms that constructs $\epsilon$-net landmarks.

% The problem with the maxmin heuristic is that, the choice of the first landmark affects the landmarks chosen later. 
% \begin{figure}[t!]
% \centering
% 	%\begin{subfigure}{\linewidth}
% 		\includegraphics[width=0.32\textwidth,trim=1.1cm 1.1cm 1.1cm 1.1cm]{dexa2/relation/epsnet_.pdf}
% 		%\caption{A 1-net}
% 		\label{fig:1net}
% 	%\end{subfigure}
% 	%\begin{subfigure}{0.3\linewidth}
% 		\includegraphics[width=0.32\textwidth,trim=1.1cm 1.1cm 1.1cm 1.1cm]{dexa2/relation/maxmin_.pdf}
% 		%\caption{A $0.9014$-net}
% 		\label{fig:maxminnet1}
% 	%\end{subfigure}
% 	%\begin{subfigure}{0.3\linewidth}
% 		\includegraphics[width=0.32\textwidth,trim=1.1cm 1.1cm 1.1cm 1.1cm]{dexa2/relation/maxmin_2.pdf}
% 		%\caption{A $\sqrt{2}$-net}
% 		\label{fig:maxminnet2}
% 	%\end{subfigure}
% 	\caption{Four landmarks are selected from 8 points on a circle at $(0,0)$ with radius $1$. Cover of each landmark is shown as a ball centered at that landmark. Pair-wise distances between landmarks shown by drawing edges with distance as weights. (left) An $1$-net constructed using algorithm ~\ref{alg:1}. (middle) Same number of points (4) is used to construct select landmarks using maxmin. The landmarks are selected in order $2>7>5>1$. The landmarks are $0.9014$-sparse. (right) Another set of $4$ landmarks chosen using maxmin. The landmarks are selected in order $7>3>1>5$. The landmarks are $\sqrt{2}$-sparse.}
% 	\label{fig:comp}
% \end{figure}

% Figure~\ref{fig:comp} illustrates a relationship between landmarks selected using $\epsilon$-net heuristic and those selected using the maxmin heuristics. Given $\epsilon$, algorithm ~\ref{alg:1} select landmarks which are at least $\epsilon$-sparse and $\epsilon$-sample. Given the choice of number of landmarks $k$, maxmin-heuristic selects landmarks that are $\delta$-sparse,$\delta$-sample  where $\delta$ is the minimum of the pairwise distances among the landmarks chosen. Figures~\ref{fig:maxminnet1} and ~\ref{fig:maxminnet2} also show that there is no guarantee on the value of $\delta$ for which the landmarks are a $\delta$-net even though same number of landmarks are chosen, which is due to the dependency of the initial point chosen by maxmin.


%We show that the above algorithm does indeed compute an $\epsilon$-net.
% \textit{Correctness of Algorithm~\ref{alg:1}.}
% The initial landmark set $\{l_1\}$ is an $\epsilon$-sparse. Suppose, the set of landmarks $\{l_1,\cdots,l_i\}$ at iteration $i$ is an $\epsilon$-sparse. The landmark $l_{i+1}$ chosen by the algorithm at iteration $i+1$ must be unmarked, which implies that $l_{i+1}$ is not in any of the sets in the family $\{B_\epsilon(l_1), \cdots, B_\epsilon(l_i)\}$. Thus, $l_{i+1}$ is at distance greater than $\epsilon$ from $\{l_1,\cdots,l_i\}$. Therefore, $\{l_1,\cdots,l_i,l_{i+1}\}$ is also $\epsilon$-sparse. If there are $k$ landmarks in $L$ at the end of the algorithm, by induction, $\forall i \in \{1,2,\cdots,k\}$,  $\{l_1,\cdots,l_{k}\}$ is $\epsilon$-sparse. Since the algorithm terminates when there is no unmarked points, every point in $P$ must be in one of the sets in the family $\{B_\epsilon(l_i): l_i \in L\}$. Hence, $\cup_{l_i \in L} B_\epsilon(l_i) = P$, and therefore, $L$ is an $\epsilon$-sample.

% \textit{Discussion.} Har-Peled and Raichel~\cite{har2015net} proposed an $O(n)$ algorithm for constructing an $\epsilon$-net of an Euclidean space. We stick with Algorithm~\ref{alg:1} as it is simpler and in practice works better for the datasets that we study.


% \section{Approximation Guarantees of $\epsilon$-net induced lazy witness complex} 
% \label{sec:theory}
% The existing landmark selection algorithms takes number of landmarks $k$ as parameter. However, the lazy witness complex the resulting landmarks induces does not come with any guarantee in terms of the quality of the topological features approximated. We have shown in section ~\ref{sec:net} that $\epsilon$-nets are already an $\epsilon$-approximation of the point-cloud. Furthermore, We want to show that the lazy witness filtration induced by the $\epsilon$-net landmarks is a good approximation to the Rips filtration on the landmarks, irrespective of the algorithms chosen to construct it. The following lemma which we state without proof establishes relation between 1-nearest neighbor of points in an $\epsilon$-net.

% \begin{lemma}
% \label{lemma:nn1}
% Let $L$ is an $\epsilon$-net landmark of point cloud $P$. 
% \begin{enumerate}
%     \item If a point $p \in P$ is a 1-nearest neighbor of a point $l \in L$, then $d(l,p) \leq \epsilon$ 
%     \item If a point $p' \in P$ is a 1-nearest neighbor of another point $p \in P$, then $d(p,p') \leq \epsilon$.
% \end{enumerate}
% \end{lemma}
% % \begin{proof}
% % \begin{enumerate}
% %     \item Suppose not and $d(l,p) > \epsilon$. As $L$ is an $\epsilon$-net,for every point $l \in L$ there exists a point $w' \in P$ such that $d(l,w') \leq \epsilon < d(l,p)$. Hence, $p$ is not a $1$-nearest neighbor of $l$, leading to contradiction.
% %     \item Suppose not and $d(p,p') > \epsilon$. Consider the $\epsilon$-ball $B_\epsilon$ containing $p \in P$, without loss of generality consider the ball to be centered at $p''$. Now, $d(p,p'') \leq \epsilon < d(p,p')$ contradicting the fact that $p'$ is the 1-nearest neighbor of $p$. 
% % \end{enumerate}
% % \end{proof}

% The following theorem shows that a lazy witness complex induced by an $\epsilon$-net landmarks is a $(1+1/\delta)$-approximation of the Rips complex on the landmarks, except beyond a certain filtration value. 
% \begin{theorem}
% \label{thm:approx}
% 	Let for some positive real $\epsilon > 0$, L be an $\epsilon$-net chosen from point cloud $P$. Let $LW_{\alpha}(P,L,\nu = 1)$ is the lazy witness complex of $L$ at filtration value $\alpha$ and $R_\alpha(L)$ is the Vietoris-Rips complex of $L$ at filtration $\alpha$.
	
% 	For some positive real $\delta > 0$, $R_{\alpha/(1+1/\delta)} \subseteq LW_\alpha(P,L,1) \subseteq R_{\alpha(1+1/\delta)}$ if filtration parameter $\alpha>\epsilon(1+\delta)$.
% \end{theorem}

% \begin{proof}	
% 	Consider a $k$-simplex $\sigma_k = [x_0x_1 \cdots x_k] \in R_{\alpha/(1+1/\delta)}$. For any edge $[x_ix_j] \in \sigma_k$, let $w_t$ be the point in $P$ that is nearest to the vertices of $[x_ix_j]$ and wlog, let that vertex be $x_j$. 
% 	Since $w_t$ is a nearest neighbor of $x_j$, by Lemma~\ref{lemma:nn1}, $d(w_t,x_j) \leq \epsilon \leq \frac{\alpha}{1+\delta}$. 
% 	Since $[x_ix_j] \in  R_{\alpha/(1+1/\delta)}$, $d(x_i,x_j) \leq \frac{\alpha}{1 + 1/\delta} = \frac{\alpha \delta}{1+\delta}$. By Triangle inequality, $d(w_t,x_i) \leq \frac{\alpha}{1+\delta} +  \frac{\alpha\delta}{1 + \delta} \leq \alpha$. Hence, $x_i$ is withing distance $\alpha$ from $w_t$. Since the distances from $w_t$ to its nearest points of $L$ are non-negative, $w_t$ is an witness to the edge $[x_ix_j]$. As a result $[x_ix_j] \in LW_\alpha(P,L,1)$. Since this is true for all $x_i,x_j \in \sigma_k$, the $k$-simplex $\sigma_k \in LW_\alpha(P,L,1)$.
	
% 	To prove the second inclusion, consider a $k$-simplex $\sigma_k = [x_0x_1 \cdots x_k] \in LW_\alpha(P,L,1)$. Therefore, for any edge $[x_ix_j]$ of $\sigma_k$ there is a witness $w \in P$ such that, $d(x_i,x_j) \leq d_N^1(w) + \alpha \leq \epsilon + \alpha \text{(by Lemma ~\ref{lemma:nn1})} \leq \frac{\alpha}{1+\delta} + \alpha \leq \frac{\alpha}{\delta} + \alpha (\text{Since } \delta > 0) \leq \alpha (1 + 1/\delta)$. Since this is true for all  $x_i,x_j \in \sigma_k$, the k-simplex $\sigma_k \in R_{\alpha(1+1/\delta)}$.  
	
% \end{proof}

% % {\color{red}{\textbf{Idea of measuring loss in wasserstein/bottleneck distance, given the loss due to lazy witness approximation}
% % \textbf{Idea of a distance measure:} Quantify 1. the loss due to lazy witness from a quantity derived from the above idea. Plus 2. the loss due to epsilon-net sampling (? how? is it already accounted for when we derive the quantity from the above idea?)}}. 

% % We state the following lemma which we use to discuss the approximation guarantees of lazy witness complex on $\epsilon$-net.

% % \begin{lemma}{Persistence Approximation Lemma~\cite[Lemma 3.2]{sparse_rips}.}
% % For any two filtrations $A = \{A_\alpha\}_{\alpha \geq 0}$ and $B = \{B_\alpha\}_{\alpha \geq 0}$, if $A_{\frac{\alpha}{c}} \subseteq B_{\alpha} \subseteq A_{c\alpha}$ for all $\alpha \geq 0$ then the
% % persistence diagram $Dgm(A)$ is a $c$-approximation to the persistence diagram $Dgm(B)$.
% % \end{lemma}

% \emph{Discussion.} In Theorem~\ref{thm:approx}, we show that the interleaving of lazy witness filtration $LW = {LW_\alpha(L)}$ and the Rips filtration $R = R_\alpha(L)$ only occurs when $\alpha > \epsilon(1+\delta)$. Hence the diagrams $Dgm(LW)$ and $Dgm(R)$ are $(1+1/\delta)$-approximations of each other. One consequence of the persistence approximation lemma is that the bottleneck distance $d_B(A,B)$ between filtrations $A$ and $B$ is bounded above by $(1+1/\delta)$. 





==> ATDA2019(cr)/background.tex <==
\section{Topological Data Analysis}\label{sec:tda}%\vspace{-.5em}
Topological data analysis is the study of computational models for efficient and effective computation of topological features, such as persistent homology classes, from different datasets, and representation of the topological features using different topological descriptors, such as persistence barcodes, for further analysis and application~\cite{edelsbrunner2010computational,otter2017roadmap}.
In this section, we represent the computational blocks of topological data analysis in Figure~\ref{fig:pipeline} and further describe each of the blocks.
\begin{figure}[!htbp]
    \centering
    \includegraphics[width=0.4\textwidth]{blocks/TDA_pipeline.pdf}
    \caption{Components of topological data analysis.}
    \label{fig:pipeline}
\end{figure}

Topological data analysis computes the topological features, such as persistent homology classes, by computing the topological objects called \emph{simplicial complex} for a given dataset. A \textbf{simplicial complex} is constructed using simplices. Formally, a \emph{$k$-simplex} is the convex-hull of $(k+1)$ data points. For instance, A 0-simplex $[v_0]$ is a single point, a 1-simplex $[v_0v_1]$ an edge, and a 2-simplex $[v_0v_1v_2]$ a filled triangle. 


\color{red}A \textbf{$k$-homology class} is an equivalent class of such $k$-simplicial complexes that cannot be reduced to a lower dimensional simplicial complex~\cite{edelsbrunner2010computational}.


In order to compute the $k$-homology classes, a practitioner does not have direct access to the underlying space of the point cloud and it is combinatorially hard to compute the exact simplicial representation of \v Cech complex~\cite{zomorodian2010fast}.
Thus, different approximations of the exact simplicial representation are proposed: \emph{Vietoris-Rips} complex~\cite{hausmann1995vietoris} and \emph{lazy witness} complex~\cite{de2004topological}.

The \textbf{Vietoris-Rips complex} $R_\alpha(D)$, for a given dataset $D$ and real number $\alpha > 0$, is an abstract simplicial complex representation consisting of such $k$-simplices, where any two points $v_i, v_j$ in any of these $k$-simplices are at distance at most $\alpha$. Vietoris-Rips complex is the best possible ($\sqrt{2}$-)approximation of the \v Cech complex, computable with present computational resources, and is extensively used in topological data analysis literature~\cite{otter2017roadmap}. Thus, we use the Vietoris-Rips complex as the baseline representation in this paper.
In the worst case, the number of simplices in the Vietoris-Rips complex grows exponentially with the number of data points~\cite{otter2017roadmap,zomorodian2010fast}. 
Lazy witness complex~\cite{de2004topological} approximates the Vietoris-Rips complex by constructing the simplicial complexes over a subset of data points $L$, referred to as the landmarks. 
% Though this approximation leads to loss of topological features, lazy witness complex captures a portion of the topological features of the underlying space depending on the choice of landmarks. 
% \vspace*{-1em}
% \begin{definition}[Lazy Witness Complex~\cite{de2004topological}]
Formally, given a positive integer $\nu$ and real number $\alpha>0$, the \textbf{lazy witness complex} $LW_\alpha(D,L,\nu)$ of a dataset $D$ is a simplicial complex over a landmark set $L$ where for any two points $v_i,v_j$ of a $k$-simplex $[v_0 v_1\cdots v_k]$, there is a point $w$ whose $(d^\nu(w) + \alpha)$-neighbourhood\footnote{$d^\nu(w)$ is the  geodesic distance from point $w \in V$ to its $\nu$-th nearest point in $L$.} contains $v_i, v_j$.
%\end{definition}\vspace{-1em}
In the worst case, the size of the lazy witness complexes grows exponentially with the number of landmarks. Less number of landmarks facilitates computational acceleration while produces a bad approximation of Vietoris-Rips with loss of topological features. Thus, the trade-off between the approximation of topological features and available computational resources dictates the choice of landmarks. We provide a quantification on such loss of topological features  which was absent in the literature.

%For a given filtration parameter $\alpha$, the Rips and lazy witness complex provide corresponding approximate simplicial complex representations.
As the value of filtration parameter $\alpha$ increases, new simplices arrive and the topological features, i.e. the homology classes, start to appear. Some of the homology classes merge with the existing classes in a subsequent simplicial complex, and some of them persist indefinitely~\cite{edelsbrunner2010computational}.
In order to capture the evolution of topological structure with scale, topological data analysis techniques construct a sequence of simplicial complex representations, called a \emph{filtration}~\cite{edelsbrunner2010computational}, for an increasing sequence of $\alpha$'s. 
In a given filtration, the persistence interval of a homology class is denoted by $[\alpha_{b},\alpha_{d})$, where $\alpha_{b}$ and $\alpha_{d}$ are the filtration values of its appearance and merging respectively. The persistence interval of an indefinitely persisting homology class is denoted as $[\alpha_{b},\infty)$.
Topological descriptors, such as barcodes~\cite{collins2004barcode}, persistence diagram~\cite{edelsbrunner2010computational}, and persistence landscapes~\cite{bubenik2015statistical}, represent persistence intervals in order to draw qualitative and quantitative inference about the topological features. Distance measures between persistent diagrams such as the q-Wasserstein and Bottleneck distance~\cite{edelsbrunner2010computational} are often used to draw quantitative inference.

==> ATDA2019(cr)/conclusion.tex <==
\section{Conclusion and Future Work}~\label{sec:conc}
We investigate the computation of persistent homologies on  weighted graphs. We extend the notion of $\epsilon$-net for point clouds to weighted graphs. We further propose an $\epsilon$-net induced lazy witness complex that leverages the $\epsilon$-net and their geodesic distances to select landmarks. 
%We show that the value of the $\epsilon$ parameter of the $\epsilon$-net provides a control on the trade-off between choice and number of landmarks and the quality of the approximate simplicial representation. 

We prove that an $\epsilon$-net of a connected graph is an $\epsilon$-approximation of its set of vertices in Hausdorff distance.
We also prove that the lazy witness complex induced by an $\epsilon$-net is a $3$-approximation of the Vietoris-Rips complex induced by the same set.
We prove the existence of an $\epsilon$-net (of a graph) of size at most $(\frac{\Delta}{\epsilon})^{O(\log{\frac{|V|}{\epsilon}})}$, where $\Delta$ is the diameter of the graph.
    
We present three algorithms for constructing an $\epsilon$-net of a graph. We comparatively and empirically evaluate the efficiency and effectiveness of the choice of landmarks that they induce for the topological data analysis of several real world graphs. The empirical performance analysis instantiates Iterative-$\epsilon$-Net as the practical and efficient choice to construct $\epsilon$-net induced lazy witness complex for graphs.

An interesting future work would be to leverage the notion of $\epsilon$-net induced lazy witness complex for faster and scalable computation of machine learning problems, such as clustering~\cite{chazal2013tomato}, deep learning~\cite{pmlr-v97-hofer19a}, kernel density estimation~\cite{carriere2017sliced}, for both graphs and point clouds.

\section*{Acknowledgement}
This work is partially supported by the National University of Singapore Institute for Data Science project WATCHA and by Singapore Ministry of Education project Janus.

==> ATDA2019(cr)/enet.tex <==
\section{$\epsilon$-net of Graphs: Definition and Analysis}
\label{sec:net_graph}
\cite{naheed2019} proposes the $\epsilon$-net induced lazy witness complex for a point cloud embedded in a Euclidean space for efficient computation of topological data analysis. In practice, the datasets may not be represented as a point cloud in a Euclidean space. The data may have different representations and non-Euclidean geometry. For instance, the dataset with contextual and relational structure is often represented using graphs. In a graphical representation of data, the vertices represent the data objects, edges represent relations among the data objects, and weights on the edges quantify the amplitude of the relation with respect to others.

In this paper, we study both weighted and unweighted simple graphs.
Since unweighted graphs are a special case of weighted graph, we construct the definitions for weighted simple graphs. A weighted simple graph~\cite{berge} $G(V,E,W)$ is a graph with a vertex set $V$, an edge set $E$, a weight function $W:V \times V \rightarrow \mathbf{R}^{+}$, and does not contain any self-edge or multiple edge. The geodesic distance $d_G(u,v)$ between a pair $u,v$ of vertices in a graph is defined as the length of the shortest path between $u$ and $v$, where the path length is defined as the sum of weights of the edges connecting the vertices $u$ and $v$~\cite{newman2004analysis}. %{\color{blue}
In this paper we treat a graph $G = (V,E,W)$ as a set $V$ endowed with the canonical metric $d_G: V \times V \rightarrow \mathbf{R}^{+}$. Thus, a weighted simple graph $G$ transforms into a metric space $(V,d_G)$.%}

As we substitute the points in the point cloud with the vertices of the graph and the Euclidean distance between points with the geodesic distance between the vertices, we adapt the components of topological data analysis for simple weighted graphs. 

%A graph $G$ is a triple $(V,E,W)$. $V$ is a finite set of objects called vertices. $E \subset V \times V$ are the edges and $W: E \rightarrow \mathbf{R}$ is a weight function associated to each edge. We assume the graph as connected for all practical purposes. The length of a path $p(u \sim v)$ from vertex $u$ to $v$ is defined as the summation $\sum_i w(e_i)$, where each edge $e_i$ is in the path. The geodesic distance $d_G(u,v)$ is the length of the path with smallest length over all paths from $u$ and $v$.

% \subsection{Landmark Selection Heuristics}\label{sec:heuristics}\vspace*{-0.5em}
% {\color{blue} Divide into three sections: existing techniques (random and maxmin), optimising the effect of the initial point, and centrality based techniques (due to different modalities degree distribution)}
% {\color{blue} In each heuristic write: what is the intuition behind the heuristics, what is the computation method, what is the benefit, what is the problem}

% Removed because of reviewers' suggestion:-
% {\color{red}As mentioned in \Cref{sec:intro}, topological data analysis of a dataset begins with the computation of simplicial complex representations. 
% Though Vietoris-Rips is the best possible approximation of the \v{C}ech complex, it incurs an exponential computational cost with respect to the number of vertices of the graph. Thus, lazy witness complex is often used as a practical solution for scalable topological data analysis.
% Computation of lazy witness complex is dependent on the selection of landmarks.
% Selection of landmarks dictates the trade-off between \textit{effectiveness}, i.e. the quality of approximation of topological features, and \textit{efficiency}, i.e. the computational cost of computing the lazy witness complex. }

$\epsilon$-cover is a construction used in topology to compute inherent properties of a given space~\cite{heinonen2012lectures}.
In this paper, we import the concept of $\epsilon$-cover to define $\epsilon$-net of a graph. We use the $\epsilon$-net of a graph as landmarks for constructing lazy witness complex on that graph. 

We show that $\epsilon$-net, as a choice of landmarks, has guarantees such as being an $\epsilon$-approximate representation of the graph, its induced lazy witness complex being a $3$-approximation of the corresponding Vietoris-Rips complex, and also bounding the number of landmarks for a given $\epsilon$. These guarantees are absent for the other existing landmark selection algorithms such as random and maxmin algorithms~\cite{silva2006selecting}.

% We propose three algorithm to construct $\epsilon$-net landmarks, as well as establish their relationship with the existing algorithms maxmin and random that further justifies the algorithms. 
%{\color{blue}{
%\subsection{Graphs}
%A graph $G$ is a triple $(V,E,W)$. $V$ is a finite set of objects called vertices. $E \subset V \times V$ are the edges and $W: E \rightarrow \mathbf{R}$ is a weight function associated to each edge. We assume the graph as connected for all practical purposes. The length of a path $p(u \sim v)$ from vertex $u$ to $v$ is defined as the summation $\sum_i w(e_i)$, where each edge $e_i$ is in the path. The geodesic distance $d_G(u,v)$ is the length of the path with smallest length over all paths from $u$ and $v$.
\vspace{-1em}
\subsection{Defining $\epsilon$-net of a Graph}\vspace{-1em}
In this paper, we consider a graph $G = (V,E,W)$ as a finite metric space $(V,d_G)$. Since there are many graphs that are neither Euclidean nor they have Euclidean embedding, we extend the definitions of neighbourhood and cover from point-set topology as follows before defining $\epsilon$-net. 
% We define the notion of $\epsilon$-neighbourhood in graph-theoretic terms that is in the core of the definitions of simplicial representations considered in this paper. 
\begin{definition}[$\epsilon$-neighbourhood]\label{def:eneighbour}
	The $\epsilon$-neighbourhood $\mathcal{N}_\epsilon(u)$ of a vertex $u \in V$ is a subset of the vertex set $V$ such that for any vertex $v \in \mathcal{N}_\epsilon(u)$ the distance $d_G(u,v) \leq \epsilon$.
\end{definition}
The notion of $\epsilon$-cover for graph generalises the geometric notion of cover using the set-theoretic notion of $\epsilon$-neighbourhood in Definition~\ref{def:eneighbour}. 
\begin{definition}[$\epsilon$-cover]
	An $\epsilon$-cover of $G$ is the finite collection $\{\mathcal{N}_{\epsilon/2}(u_i) \}$ of $\epsilon/2$-neighbourhoods of vertices in $G$ such that $\cup_i \mathcal{N}_\frac{\epsilon}{2}(u_i) = V$.
\end{definition}
By triangle inequality, any set in the $\epsilon$-cover has the property that two vertices $u,v$ in the cover have geodesic distance $d_G(u,v)\leq \epsilon$. We differentiate an $\epsilon$-cover from the set of vertices whose $\frac{\epsilon}{2}$-neighbourhood determines that cover by defining $\epsilon$-sample. 
\begin{definition}[$\epsilon$-sample]
A set $L = \{u_1,u_2,\dots,u_{|L|}\} \subseteq V$ is an $\epsilon$-sample of graph $G$ if the collection $\{\mathcal{N}_{\epsilon}(u_i):u_i\in L\}$ of $\epsilon$-neighbourhoods covers $G$ i.e. $\cup_i \mathcal{N}_\epsilon(u_i) = V$.
\end{definition}
$\epsilon$-neighbourhoods may intersect, which is not an intended property if we want to decrease the size of the $\epsilon$-sample. We combine the notion of $\epsilon$-cover with the notion of $\epsilon$-sparsity to define $\epsilon$-net.
%\begin{definition}[$\epsilon$-sample]
%A set $L = \{u_1,u_2,\dots,u_{|L|}\} \subseteq V$ is an $\epsilon$-sample of graph $G$ if the collection $\{N_{\epsilon}(u_i):u_i\in L\}$ of $\epsilon$-neighborhood of radius $\epsilon$ covers $G$ , i.e. $G = G_{\cup_{u_i \in L} N_\epsilon(u_i)}$.
%\end{definition}
%According to the definition of $\epsilon$-sample, $V$ itself is an $0$-sample of the graph $G$. For decreasing further computational expense, it is desirable to have an $\epsilon$-sample that contains less number of points and thus, sparse. An $\epsilon$-sparse subset of $V$ is a subset where any two vertices are at least $\epsilon$ geodesic apart from each other in graph $G$.\vspace*{-.2em}
\begin{definition}[$\epsilon$-sparse]
A set $L = \{u_1,u_2,\dots,u_{|L|}\} \subset V$ is $\epsilon$-sparse if for any distinct $u_i,u_j \in L$,  $d_G(u_i,u_j) > \epsilon$ in graph $G$.
\end{definition}
An $\epsilon$-net of graph $G$ is such a subset of $V$ which is both an $\epsilon$-sample of $G$ and $\epsilon$-sparse. The $\epsilon$-net while considered as the landmark set $L$ induces a metric subspace $(L,d_L)$ of the metric space of the graph of $(V,d_G)$, where $d_L$ is the metric induced on set $L$ by the geodesic metric $d_G$.
\begin{definition}[$\epsilon$-net] 
A subset $L \subset V$ is an $\epsilon$-net of $G$ if $L$ is $\epsilon$-sparse and an $\epsilon$-sample of $G$.
\end{definition}
\textbf{Relating $\epsilon$-net and Other Graph Theoretic Concepts.}
The definition of $\epsilon$-net on graphs generalises the notion of independent set and dominating set for undirected graphs~\cite{berge}. Any $1$-net of an undirected graph $G = (V,E)$ is an independent set of $G$ and vice versa.  Any minimal cardinality $1$-net of $G$ is a dominating set of $G$, and vice versa.\vspace*{-1.3em}

% $\epsilon$-nets are not unique.

\subsection{Analysing Properties of $\epsilon$-net of a Graph}
\label{subsec:prop}
$\epsilon$-net of a simple, weighted, connected graph comes with approximation guarantees irrespective of its algorithmic construction.
In this section, we provide following three analysis of $\epsilon$-net:
\begin{enumerate}
    \item An $\epsilon$-net of a connected graph is an $\epsilon$-approximation of its set of vertices in Hausdorff distance.
    \item The lazy witness complex induced by an $\epsilon$-net is a $3$-approximation of the Vietoris-Rips complex induced by the same set.
    \item For a graph of diameter $\Delta$, there exists an $\epsilon$-net of  of size at most $(\frac{\Delta}{\epsilon})^{O(\log{\frac{\abs{V}}{\epsilon}})}$.
\end{enumerate} 
%\textbf{True for planar graph in D-dimensional euclidean space.May change for general graphs} 
%Here, we establish the first two approximation guarantees of $\epsilon$-net theoretically. %In section ~\ref{sec:experiment} we validate the last two properties empirically for the proposed  algorithms for constructing $\epsilon$-nets.

\paragraph{Graph Approximation Guarantee of an $\epsilon$-net.}\label{subsec:hausdorff}
We use Lemma \ref{lemma:esampleg} to prove that the $\epsilon$-net of a graph $G = (V,E,W)$ is an $\epsilon$-approximation of $V$ in Hausdorff metric (Theorem \ref{thm:hausdorff}). Lemma \ref{lemma:esampleg} follows from the $\epsilon$-sample property of an $\epsilon$-net.
\begin{lemma}\label{lemma:esampleg}
Let $L$ be an $\epsilon$-net of graph $G$. For any vertex $v \in V$, there exists a point $u \in L \subseteq V$ such that the geodesic distance $d_G(u,v) \leq \epsilon$
\end{lemma}
\begin{proof}
Since $V = \cup_{u \in L}\mathcal{N}_\epsilon(u)$, for any vertex $v \in V$ there exists an $u \in L$ such that $v \in \mathcal{N}_\epsilon(u)$. 
%Pick $u'$ as $u$. 
As $v \in \mathcal{N}_\epsilon(u)$, by definition of $\epsilon$-neighbourhood, the length of the shortest path from $v$ to $u$ is at most $\epsilon$, i.e. $d_G(u,v) \leq \epsilon$.
\end{proof}

% {\color{red}{We use the definition of graph hausdorff distance from~\cite{graph_hausdorff} to show the $\epsilon$-approximation property of $\epsilon$-net induced subgraph.
% \begin{definition}[Graph Hausdorff distance.~\cite{graph_hausdorff}]
% Need to read that paper.
% \end{definition}


\begin{theorem}
\label{thm:hausdorff}
The Hausdorff distance between  $(V,d_G)$ and its $\epsilon$-net induced subspace $(L,d_L)$ is at most $\epsilon$.
\end{theorem}
\begin{proof}
 For any $u \in L \subseteq V$, there exists a vertex $v \in V$ such that $d_G(u,v) \leq \epsilon$, by definition of $\epsilon$-neighbourhood. Hence,
%  $\min_{u\in L}{d_G(u,v)} \leq \epsilon$, and 
$\max_{L}{\min_{V}{d_G(u,v)}} \leq \epsilon$. 
% For any $v \in V$, there exists a vertex $u \in L$ such that $d_G(u,v) \leq \epsilon$, by Lemma~\ref{lemma:esampleg}. 
By Lemma~\ref{lemma:esampleg},  $\max_{V}{\min_{L}{d_G(u,v)}} \leq \epsilon$. Since the Hausdorff distance $d_H(V,L)$  is defined as the maximum of $\max_{L} \min_{V}{d_G(u,v)}$ and $\max_{V}{\min_{L}{d_G(u,v)}}$, therefore $d_H(V,L)$ is upper bounded by $\epsilon$.
\end{proof}

\paragraph{Topological Approximation Guarantee of an $\epsilon$-net induced Lazy witness complex on graphs.} 
\label{subsec:theory}
% The existing landmark selection algorithms (described in section ~\ref{sec:construction}) takes number of landmarks $k$ as parameter. However, the lazy witness complex the resulting landmarks induces does not come with any guarantee in terms of the quality of the topological features approximated. 
In addition to an $\epsilon$-net being an $\epsilon$-approximation of the space $(V,d_G)$, we prove that the lazy witness complex induced by the $\epsilon$-net, as landmarks, is a good approximation (\Cref{thm:approx}) to the Vietoris-Rips complex on the same set of vertices. This approximation ratio is independent of the algorithm constructing the $\epsilon$-net. As a step towards \Cref{thm:approx}, we state \Cref{lemma:nn1}. \Cref{lemma:nn1} is implied by the definition of the lazy witness complex and $\epsilon$-sample. \Cref{lemma:nn1} establishes the relation between 1-nearest neighbour of points in an $\epsilon$-net.

\begin{lemma}\label{lemma:nn1}
If $L$ is an $\epsilon$-net of $(V,d_G)$, the distance $d_G(u,v)$ from any vertex $u \in L$ to its 1-nearest neighbour $v \in V$ is at most $\epsilon$.
% \begin{enumerate}
%     \item If a point $p \in V$ is a 1-nearest neighbor of a point $l \in L$, then $d(l,p) \leq \epsilon$ 
%     \item If a point $p' \in V$ is a 1-nearest neighbor of a point $p \in V$, then $d(p,p') \leq \epsilon$.
% \end{enumerate}
\end{lemma}
% \begin{proof}
% \begin{enumerate}
%     \item Suppose not and $d(l,p) > \epsilon$. As $L$ is an $\epsilon$-net,for every point $l \in L$ there exists a point $w' \in V$ such that $d(l,w') \leq \epsilon < d(l,p)$. Hence, $p$ is not a $1$-nearest neighbor of $l$, leading to contradiction.
%     \item Suppose not and $d(p,p') > \epsilon$. Consider the $\epsilon$-ball $B_\epsilon$ containing $p \in V$, without loss of generality consider the ball to be centered at $p''$. Now, $d(p,p'') \leq \epsilon < d(p,p')$ contradicting the fact that $p'$ is the 1-nearest neighbor of $p$. 
% \end{enumerate}
% \end{proof}
\Cref{thm:approx} shows that a lazy witness complex induced by an $\epsilon$-net landmarks is a $3$-approximation of the Vietoris-Rips complex on the landmarks beyond a certain value of the filtration parameter. 

\begin{theorem}
	\label{thm:approx}
	If $L$ is an $\epsilon$-net of the point cloud $V$ for $\epsilon \in \mathbf{R}^+$, $LW_{\alpha}(V,L,\nu = 1)$ is the lazy witness complex of $L$ at filtration value $\alpha$, and $R_\alpha(L)$ is the Vietoris-Rips complex of $L$ at filtration $\alpha$, 
	$R_{\alpha/3}(L) \subseteq LW_\alpha(V,L,1) \subseteq R_{3\alpha}(L)$ for $\alpha \geq 2\epsilon$.
\end{theorem}\vspace{-1.5em}
\begin{proof}	
	In order to prove the first inclusion, consider a $k$-simplex $\sigma_k = [x_0 \cdots x_k]$ $\in R_{\alpha/3}(L)$. For any edge $[x_ix_j] \in \sigma_k$, let $w_t$ be the point in $V$ that is nearest to the vertices of $[x_ix_j]$. Without loss of generality, let that vertex be $x_j$. 
	Since $w_t$ is the nearest neighbour of $x_j$, by Lemma~\ref{lemma:nn1}, $d_G(w_t,x_j) \leq \epsilon \leq \frac{\alpha}{2}$. 
	Since $[x_ix_j] \in  R_{\alpha/3}$, $d_G(x_i,x_j) \leq \frac{\alpha}{3} < \frac{\alpha}{2}$. By triangle inequality, $d_G(w_t,x_i) \leq \frac{\alpha}{2} +  \frac{\alpha}{2} \leq \alpha$. Hence, $x_i$ is within distance $\alpha$ from $w_t$. The $\alpha$-neighbourhood of point $w_t$ contains both $x_i$ and $x_j$. 
	Since $d^1(w_t) > 0$, the $(d^1(w_t) + \alpha)$-neighbourhood of $w_t$ also contains $x_i,x_j$. Therefore, $[x_ix_j]$ is an edge in $LW_\alpha(V,L,1)$. Since the argument is true for any $x_i,x_j \in \sigma_k$, the $k$-simplex $\sigma_k \in LW_\alpha(V,L,1)$.
	
	In order to prove the second inclusion, consider a $k$-simplex $\sigma_k = [x_0x_1 \cdots x_k]$ $\in LW_\alpha(V,L,1)$. Therefore, by definition of lazy witness complex, for any edge $[x_ix_j]$ of $\sigma_k$ there is a witness $w \in V$ such that, the $(d^1(w) + \alpha)$-neighbourhood of $w$ contains both $x_i$ and $x_j$. Hence, $d_G(w,x_i) \leq d^1(w) + \alpha \leq \epsilon + \alpha$  (by Lemma ~\ref{lemma:nn1})$\leq 3\alpha/2$. Similarly, $d_G(w,x_j) \leq 3\alpha/2$. By triangle inequality, $d_G(x_i,x_j) \leq 3\alpha$. Therefore, $[x_ix_j]$ is an edge in $R_{3\alpha}(L)$. Since the argument is true for any  $x_i,x_j \in \sigma_k$, the k-simplex $\sigma_k \in R_{3\alpha}(L)$.  
\end{proof}

\emph{Discussion.} Theorem~\ref{thm:approx} implies that the interleaving of lazy witness filtration $LW = {LW_\alpha(L)}$ and the Vietoris-Rips filtration $R = R_\alpha(L)$ occurs when $\alpha > 2\epsilon$. As a consequence, their corresponding partial persistence diagrams $Dgm_{>2\epsilon}(LW)$ and $Dgm_{>2\epsilon}(R)$ are $3\log{3}$-approximations of each other in log-scale, by the persistence approximation lemma~\cite{sparse_rips}. In \Cref{sec:experiment}, we empirically validate this bound for the lazy witness complex induced by the $\epsilon$-net landmarks.

\paragraph{Size of an $\epsilon$-net.} 
We prove an upper bound on the size of an $\epsilon$-net of a connected unweighted graph using the \emph{doubling dimension}.

The doubling dimension~\cite{gupta2003bounded}  of a metric space $M = (X,d)$ is the smallest positive number $D$ such that any $\epsilon$-neighbourhood in $M$ can be covered by $2^D$ number of $\frac{\epsilon}{2}$-neighbourhoods. %A metric space $M = (X,d)$ having doubling dimension $D$ means that, for any $\epsilon$-neighborhood, there exists a collection of $\epsilon/2$-neighborhoods of cardinality $2^{D}$ covering $X$, and it is the smallest collection with such property. 
A metric space is called \emph{doubling} if its doubling dimension is bounded. The space $(V,d_G)$ is a doubling metric space.

% Karger and Ruhl~\cite{karger2002finding} considered a notion of dimension based on the counting measure in finite metric spaces: Let $K$ be the smallest constant such that $|\mathcal{N}(x,2\epsilon)| \leq K|\mathcal{N}(x,\epsilon)|$ for all $x \in X, \epsilon \geq 0$. $K$ is the KR-constant of $X$ and $\log_2(K)$ is the KR-dimension of $X$, denoted as $D_{KR}(X)$

% Gupta et. al. proved that, for any finite metric space $(X,d)$, its doubling dimension $D(X) \leq 4.D_{KR}(X)$. 

Gupta et. al.~\cite{gupta2003bounded} showed that the doubling dimension $D(G)$ of an unweighted connected graph $G$ is related to its local density. The local density of an unweighted connected graph $G$, denoted $\beta(G)$, is the smallest value $\beta$ such that $\abs{\mathcal{N}_\epsilon(v)} \leq \beta \epsilon$, for all $v \in V$ and $\epsilon \in \mathbf{N}$. To be precise the doubling dimension $D(G) \leq 4 \log(2\beta(G))$~\cite{gupta2003bounded}. We use this result along with the following lemma to prove bound on the size of an $epsilon$-net of an unweighted graph in Theorem~\ref{thm:epsnetsz}.

\begin{lemma}
\label{lemma:doubling}
For any connected unweighted graph $G$ of diameter $\Delta$ and doubling dimension $D(G)$, there exists an $\epsilon$-net of size at most $(\frac{\Delta}{\epsilon})^{D(G)}$ where $\Delta \geq \epsilon \geq 1$
\end{lemma}\vspace{-1.5em}
\begin{proof}
Let $\Delta$ be the diameter of an unweighted graph $G$ of doubling dimension $D(G)$. Thus, $V$ (a $\Delta$-neighbourhood) can be covered by $2^{D(G)}$ number of $\Delta/2$-neighbourhoods. Each $\Delta/2$-neighbourhood can be covered by $2^{D(G)}$ number of $\Delta/4$-neighbourhoods. Thus $V$ can be covered by $2^{2D(G)}$ number of $\Delta/4$-neighbourhoods. Repeating this $\log_2(\frac{\Delta}{\epsilon})$-times, we get that $V$ can be covered by $2^{D(G)\log_2(\frac{\Delta}{\epsilon})}$ number of $\epsilon$-neighbourhoods. Each of the $\epsilon$-neighbourhoods contain at most one $\epsilon$-net-landmark. Hence, there exists an $\epsilon$-net of size $(\frac{\Delta}{\epsilon})^{D(G)}$ for any connected, unweighted graph $G$.
\end{proof}\vspace{-1.5em}
\input{algo_1.tex}
% \textit{Bounds on $D(G)$ for graphs:}
\begin{theorem}
\label{thm:epsnetsz}
    For any connected unweighted graph $G = (V,E)$ of diameter $\Delta$, there exists an $\epsilon$-net of size at most $(\frac{\Delta}{\epsilon})^{O(\log(\frac{\abs{V}}{\epsilon}))}$ 
\end{theorem}\vspace{-1.5em}
\begin{proof}
In a connected unweighted graph $G$, the size $\abs{\mathcal{N}_\epsilon(v)}$ of $\epsilon$-neighbourhood of a vertex $v$ is greater than $\epsilon$ for $\Delta \geq \epsilon \geq 1$.
Thus, local density $\beta(G) > 1$. We observe that $\max_v \abs{\mathcal{N}_\epsilon(v)} < \abs{V}$. Thus, $\beta(G) = \max_{v,\epsilon} \frac{\abs{\mathcal{N}_\epsilon(v)}}{\epsilon}$ is at most $\frac{\abs{V}}{\epsilon}$. Applying the result from Gupta et.al.~\cite{gupta2003bounded}, the doubling dimension $D(G) \leq 4 \log(\frac{\abs{V}}{\epsilon})$. The rest  follows from~\Cref{lemma:doubling}.

\end{proof}
% The size of an $\epsilon$-net depends on $\epsilon$, the diameter of the point-cloud and the dimension of the underlying space~\cite{krauthgamer2004navigating,har2006fast}. If a point cloud $V \subset \mathbf{R}^D$ has diameter $\Delta$, the size of an $\epsilon$-net is $(\frac{\Delta}{\epsilon})^{\theta(D)}$~\cite{krauthgamer2004navigating}. Therefore, the size of an $\epsilon$-net does not depend on the size of the point cloud. In section~\ref{sec:experiment}, we empirically validate this bound for the $\epsilon$-net landmarks generated by the proposed algorithms. The concept of $\epsilon$-net along with its approximation guarantees leads to the question of its algorithmic construction as landmarks.

% Seems like there is no upper bound for $m$ in general weighted graphs. For unweighted graphs, m is related to the local density of the graph. Given an unweighted connected graph $G = (V, E)$, the local density of $G$, denoted $\beta(G)$, is the smallest value $\beta$ such that $|N_r(v)| \leq \beta r$, for all $v \in V$, $r > 0$. It can be shown that $m \leq 4(\log{\beta(G)} + 1)$. From practical point of view, the diameter of the graphs considered here is at most 1, due to scaling. Hence, the size of $\epsilon$-net of an unweighted graph in our dataset is at most $(1/\epsilon)^{O(\log{\beta(G)})}$
% }

% For $\epsilon > 0$, the size of an $\epsilon$-net depends on $\epsilon$, diameter of the dataset and the doubling dimension of the underlying space. Suppose $(X,d)$ is a metric space with aspect ratio $\Delta$ and doubling dimension $m$.  The doubling dimension of a metric space is the smallest $\lambda$ such that any ball of radius $r$ can be covered by $2^\lambda$ balls of radius $r/2$. Then $|X| \leq \Delta^{O(m)}$. A corollary:- If the diameter of a metric space $(X,d)$ is $Diam(X)$ and doubling dimension is $m$, the size of an $\epsilon$-net is  $(Diam(X)/\epsilon)^{O(m)}$. The doubling dimension $m$ of euclidean space $\mathbf{R}^D$ is $\Theta(D)$, and for $\mathbf{R}$ and $\mathbf{R}^2$, $m = 1$ and $m = log_2(7)$ respectively. For $n \geq 7$, $m \leq Dlog(2)$
% $\epsilon$-nets of a metric space always exists~\cite{heinonen2012lectures}.


==> ATDA2019(cr)/introduction.tex <==
\section{Introduction}\label{sec:intro}
\textbf{Topological data analysis} (TDA)~\cite{carlssontda,otter2017roadmap} involves computation of topological features of datasets, such as persistent homology classes, and the representation of these topological features using such topological descriptors as persistence barcodes~\cite{edelsbrunner2010computational}.
In this section, we elaborate the computational blocks of topological data analysis as shown in Figure~\ref{fig:pipeline}. %and further describe each of the blocks.

\textbf{Simplicial Complex.} Topological data analysis computes the topological features of a dataset, such as persistent homology classes, by computing the topological objects called \emph{simplicial complex}. A \textbf{simplicial complex} is constructed using simplices. Formally, a \emph{$k$-simplex} is the convex-hull of $(k+1)$ data points. For instance, a 0-simplex $[v_0]$ is a single point, a 1-simplex $[v_0v_1]$ is an edge, and a 2-simplex $[v_0v_1v_2]$ is a filled triangle. 
A \textbf{$k$-homology class} is an equivalent class of such $k$-simplicial complexes that cannot be reduced to a lower dimensional simplicial complex~\cite{edelsbrunner2010computational}.

% \textbf{Formal introduction:} The set of $k$-simplices of a simplicial complex with mod 2 addition operation forms a group called \textit{Chain group} $C_k$. The elements in $C_k$ are called $k$-chains. The \textit{boundary map} $\partial_k: C_k(\mathcal{K})  \rightarrow C_{k-1}(\mathcal{K})$ is a homomorphism defined as
% $\partial_k(c_k) = \sum_{\sigma \in c_k} \partial(\sigma)$ where $\partial(\sigma)$ is the mod 2 sum of $(k-1)$-faces of $\sigma$. A \textit{$k$-cycle} $z_k$ is a $k$-chain such that $\partial_k(z_k) = 0$. The set of $k$-cycles forms a subgroup of $C_k(\mathcal{K})$ called the \textit{Cycle group} $Z_k$. Furthermore, A $k$-chain $b_k$ is a \textit{k-boundary} iff there exists some $c_{k+1}$ such that $\partial_{k+1}(c_{k+1}) = b_k$. The set of $k$-boundaries forms a subgroup of $C_k(\mathcal{K})$ called the \textit{Boundary group} $B_k$. The $k$-th homology group $H_k$ is the quotient group $Z_k/B_k$. An element in the $k$-th homology group is an equivalent class of $k$-cycles called the $k$-homology class. Two $k$-cycles belong to the same class if there difference is a $k$-boundary. Geometrically, elements of $H_0$,$H_1$ and $H_2$ are the connected components, cycles and voids in the simplicial complex.
In order to compute the $k$-homology classes, a practitioner does not have direct access to the underlying space of the point cloud and it is combinatorially hard to compute the exact simplicial representation of \v{C}ech complex~\cite{zomorodian2010fast}.
Thus different approximations of the exact simplicial representation are proposed: \emph{Vietoris-Rips} complex~\cite{vietoris1927hoheren} and \emph{lazy witness} complex~\cite{de2004topological}.

% The computation of persistent homologies from simplicial representations such as the Vietoris-Rips~\cite{vietoris1927hoheren} and the \v{C}ech~\cite{edelsbrunner2010computational} complexes do not efficiently scale to large point clouds. We elaborate them further in the following paragraphs.
\begin{figure}[t!]
    \centering
    \includegraphics[width=0.8\textwidth]{blocks/TDA_pipeline.pdf}\vspace{-.5em}
    \caption{Components of topological data analysis.}\vspace{-3em}
\end{figure}\label{fig:pipeline}

% \textbf{Approximate Simplicial Representations.} In order to compute the $k$-homology classes, a practitioner does not have direct access to the underlying space of the point cloud and it is combinatorially hard to compute the exact simplicial representation of \v{C}ech complex~\cite{zomorodian2010fast}. Vietoris-Rips complex~\cite{vietoris1927hoheren} is a $\sqrt{2}$-approximation of the \v{C}ech complex. The \textbf{Vietoris-Rips complex} $R_\alpha(D)$, for a given dataset $D$ and real number $\alpha > 0$, is an abstract simplicial complex representation consisting of such $k$-simplices, where any two points $u, v$ in any of these $k$-simplices are at distance at most $\alpha$. Vietoris-Rips complex is the best possible ($\sqrt{2}$-)approximation of the \v{C}ech complex, computable with present computational resources, and is extensively used in topological data analysis literature~\cite{otter2017roadmap}. Thus, we use the Vietoris-Rips complex as the \emph{baseline representation} in this paper. In the worst case, the number of simplices in the Vietoris-Rips complex grows exponentially with the number of data points~\cite{otter2017roadmap,zomorodian2010fast}. 

% Since homology computation from simplicial representations such as the Vietoris-Rips and the \v{C}ech complexes do not efficiently scale to large point clouds~\cite{otter2017roadmap}, it is therefore meaningful to devise other approximate representations~\cite{gic,sparse_rips} and evaluate the trade-off between their efficiency and effectiveness. The lazy witness complex~\cite{de2004topological} economically defines such a representation using only a few selected points, called \emph{landmarks}.

% % Thus, different approximations of the exact simplicial representation are proposed: \emph{Vietoris-Rips} complex and \emph{lazy witness} complex~\cite{de2004topological}.

% % Though this approximation leads to loss of topological features, lazy witness complex captures a portion of the topological features of the underlying space depending on the choice of landmarks. 
% % \vspace*{-1em}
% % \begin{definition}[Lazy Witness Complex~\cite{de2004topological}]
% Formally, given a positive integer $\nu$ and a real number $\alpha>0$, the \textbf{lazy witness complex} $LW_\alpha(D,L,\nu)$ of a dataset $D$ is a simplicial complex over a landmark set $L$ where for any two points $v_i,v_j$ of a $k$-simplex $[v_0 v_1\cdots v_k]$, there is a point $w$ whose $(d^\nu(w) + \alpha)$-neighborhood contains $v_i, v_j$. $d^\nu(w)$ is the distance from point $w \in V$ to its $\nu$-th nearest point in the landmark set $L$.
% %\end{definition}\vspace{-1em}
% In the worst case, the size of the lazy witness complexes grows exponentially with the number of landmarks. Less number of landmarks facilitates computational acceleration while produces a bad approximation of Vietoris-Rips with loss of topological features. Thus, the trade-off between the approximation of topological features and available computational resources dictates the choice of landmarks. \emph{We provide a quantification on such loss of topological features that was absent in the literature.}

\textbf{Approximate Simplicial Representations.} 
% Researchers devise approximate representations~\cite{gic,sparse_rips} and evaluate the trade-off between their efficiency and effectiveness. 
%The lazy witness complex~\cite{de2004topological} economically defines such a representation using only a few selected points, called \emph{landmarks}.
% In order to compute the $k$-homology classes, a practitioner does not have direct access to the underlying space of the point cloud and it is combinatorially hard to compute the exact simplicial representation of \v{C}ech complex~\cite{zomorodian2010fast}.
% Thus, different approximations of the exact simplicial representation are proposed: \emph{Vietoris-Rips} complex and \emph{lazy witness} complex~\cite{de2004topological}.
The \textbf{Vietoris-Rips complex} $R_\alpha(D)$, for a given dataset $D$ and real number $\alpha > 0$, is an abstract simplicial complex representation consisting of such $k$-simplices, where any two points $u, v$ in any of these $k$-simplices are at distance at most $\alpha$. Vietoris-Rips complex is the best possible ($\sqrt{2}$-)approximation of the \v{C}ech complex, computable with present computational resources, and is extensively used in topological data analysis literature~\cite{otter2017roadmap}. Thus, we use the Vietoris-Rips complex as the \emph{baseline representation} in this paper.
In the worst case, the number of simplices in the Vietoris-Rips complex grows exponentially with the number of data points~\cite{zomorodian2010fast}. 

Lazy witness complex~\cite{de2004topological} approximates the Vietoris-Rips complex by constructing the simplicial complexes over a subset of data points $L$, referred to as the landmarks. 
% Though this approximation leads to loss of topological features, lazy witness complex captures a portion of the topological features of the underlying space depending on the choice of landmarks. 
% \vspace*{-1em}
% \begin{definition}[Lazy Witness Complex~\cite{de2004topological}]
Formally, given a positive integer $\nu$ and a real number $\alpha>0$, the \textbf{lazy witness complex} $LW_\alpha(D,L,\nu)$ of a dataset $D$ is a simplicial complex over a landmark set $L$ where for any two points $v_i,v_j$ of a $k$-simplex $[v_0 v_1\cdots v_k]$, there is a point $w$ whose $(d^\nu(w) + \alpha)$-neighbourhood contains $v_i, v_j$. $d^\nu(w)$ is the  geodesic distance from point $w \in L$ to its $\nu$-th nearest point in the landmark set $L$.
%\end{definition}\vspace{-1em}
In the worst case, the size of the lazy witness complexes grows exponentially with the number of landmarks. Less number of landmarks facilitates computational acceleration while produces a bad approximation of Vietoris-Rips with loss of topological features. Thus, the trade-off between the approximation of topological features and available computational resources dictates the choice of landmarks. \emph{We provide a quantification on such loss of topological features that was absent in the literature.}

%For a given filtration parameter $\alpha$, the Rips and lazy witness complex provide corresponding approximate simplicial complex representations.
\textbf{Filtration and Representation of Topological Features.} As the value of filtration parameter $\alpha$ increases, new simplices arrive and the topological features, i.e. the homology classes, start to appear. Some of the homology classes merge with the existing classes in a subsequent simplicial complex, and some of them persist indefinitely~\cite{edelsbrunner2010computational}.
In order to capture the evolution of topological structure with scale, topological data analysis techniques construct a sequence of simplicial complex representations, called a \emph{filtration}~\cite{edelsbrunner2010computational}, for an increasing sequence of $\alpha$'s. 
In a given filtration, the persistence interval of a homology class is denoted by $[\alpha_{b},\alpha_{d})$, where $\alpha_{b}$ and $\alpha_{d}$ are the filtration values of its appearance and merging respectively. The persistence interval of an indefinitely persisting homology class is denoted as $[\alpha_{b},\infty)$.
Topological descriptors, such as barcodes~\cite{collins2004barcode}, persistence diagram~\cite{edelsbrunner2010computational}, and persistence landscapes~\cite{bubenik2015statistical}, represent persistence intervals in order to draw qualitative and quantitative inference about the topological features. Distance measures between persistent diagrams such as the q-Wasserstein and Bottleneck distance~\cite{edelsbrunner2010computational} are often used to draw quantitative inference.

\textbf{Graph Topological Data Analysis.} Topological data analysis (TDA)~\cite{carlssontda} traditionally considers a point cloud in a Euclidean space. In many situations, however, data is available in the form of a weighted graph. Conveniently, the vertices of the graph with the geodesic distance define a metric space. This metric space is amenable to topological data analysis. This fact does not depend on whether the graph is embeddable in a Euclidean space or not. Though the metric space induced by a graph provides a different structure than point clouds to investigate, this metric space bears the similar issues of scalable construction of representations as well as similar approximate representations, filtrations, and topological descriptors. This motivated us to exploit the generalisability of topological data analysis and to extend the $\epsilon$-net induced lazy witness complexes~\cite{naheed2019} to graphs.

\textbf{Our Contributions.}
We investigate the computation of persistent homologies on a weighted graph. In Section~\ref{sec:net_graph}, we present a lazy witness complex approach leveraging the notion of $\epsilon$-net that we adapt to weighted graphs and their geodesic distance to select landmarks. We show that the $\epsilon$ parameter of the $\epsilon$-net gives a control on the trade-off between choice and number of landmarks and the quality of the approximate simplicial representation. 

In \Cref{subsec:prop}, we prove that an $\epsilon$-net is an $\epsilon$-approximate representation of the point cloud with respect to the Hausdorff distance. We prove that the lazy witness complex induced by an $\epsilon$-net, as a choice of landmarks, is a $3$-approximation of the induced Vietoris-Rips complex.
% $\epsilon$-net allows us to provide such approximation guarantees for lazy witness complex  which was absent in the literature.

In \Cref{sec:algos}, we present three algorithms, namely Greedy-$\epsilon$-net, Iterative-$\epsilon$-net, and SPTpruning-$\epsilon$-net, for constructing an $\epsilon$-net of a graph. In Section~\ref{sec:experiment}, we comparatively and empirically evaluate the efficiency and effectiveness of the choice of landmarks that they induce for the topological data analysis of several real-world graphs. 
%Furthermore, we demonstrate and evaluate the application of $\epsilon$-net induced lazy witness complex to the graph clustering.

In Section~\ref{sec:conc}, we summarise the findings and the future directions of research that $\epsilon$-net opens up for graph topological data analysis.
%\end{section}



==> ATDA2019(cr)/relatedworks.tex <==
\begin{section}{Related Works}
% {\color{red} Justify why one would apply TDA on Graphs - Relation to assortitavity, k-core etc. Some paper among the ones above has discussed it}
\textbf{Graph TDA.} Existing applications of TDA to graphs focus on characterizing networks using features computed from persistence homology classes. \cite{Carstens2013} and \cite{petri2013topological} computed persistence homology at dimension 0, 1, and 2 of the clique filtration to study weighted collaboration networks (size $\sim$36000) and weighted networks from different domains (size $\sim$54000) respectively. 
In biology domain, \cite{duman2018gene} clustered gene co-expression networks (size $\sim$400) based on distances between Vietoris-Rips persistence diagram computed on each network. 
\cite{lee2011discriminative} studied Vietoris-Rips filtration of the functional brain networks computed on $\sim$100 region of interests (points) in human brains with different clinical disorders. They focus on homology classes at dimension 0 and 1. A related line of work regarding the topology on graphs involves graphs derived as a representation of point-cloud data (e.g. the neighbourhood graph) and their usage in data clustering~\cite{chazal2013tomato} and inference of global topology from local information~\cite{l-tda}. 

\textbf{Approximate Simplicial Complexes.} 
Computational infeasibility of constructing the \v{C}ech complex and Vietoris-Rips complex motivates the development of approximate simplicial representations such as the lazy witness complexes, sparse-Rips complex~\cite{sparse_rips} and graph induced complex (GIC)~\cite{gic}.  

\textbf{Applications of $\epsilon$-net.} The concept of $\epsilon$-net is a standard concept in analysis and topology~\cite{heinonen2012lectures} originating from the idea of $(\delta, \epsilon)$-limits formulated by Cauchy. $\epsilon$-net are sets in a metric space that covers the whole space and are well-separated. 
% In order to avoid confusion, we emphasise that the term `$\epsilon$-net' used in this paper is different from the same term used in learning theory~\cite{vcdimension} and computational geometry~\cite{enet}.
Nets have been used in nearest-neighbour search~\cite{krauthgamer2004navigating}. 
\cite{guibas2008reconstruction} used $\epsilon$-net for manifold reconstruction.
Graph induced complex~\cite{gic} uses the cliques in the neighbourhood graph to construct simplcial complex over an $\epsilon$-net. 

\cite{har2006fast} proposed net-tree data structure to represent $\epsilon$-nets at all scales of $\epsilon$. Net-tree is used to construct approximate well-separated pair decompositions~\cite{har2006fast} and approximate geometric spanners~\cite{har2006fast}. Sparse-Rips filtration~\cite{sparse_rips} constructs a net-tree on the point-cloud to decide which neighbouring points to delete.  
Contrary to Sheehy~\cite{sparse_rips}, we use $\epsilon$-net to select a fixed subset of points, called landmarks, and compute persistent homology using them.
\end{section}

==> ATDA2019(cr)/results.tex <==
%\vspace{-.5em}
\section{Performance Analysis}\label{sec:experiment}\vspace{-.5em}
In this section, we experimentally and comparatively analyse the performance of the three proposed algorithms to compute an $\epsilon$-net of graphs. We discuss the effectiveness and efficiency of the algorithms and also validate that the $\epsilon$-net computed by any of these algorithms satisfy being $3$-approximation of the Vietoris-Rips complex.
\vspace{-1em}\subsection{Datasets}\vspace{-.5em}
%\textbf{For efficiency and effectiveness validation:}
We evaluate the performance of our algorithms using two real-world datasets. The dataset Power~\cite{konect:duncan98} is an unweighted graph of US Power-grid (4941 vertices, 6594 edges, diameter 46).
Celegans~\cite{badhwar2015control} is a weighted graph of Celegans worm's frontal neural network (297 vertices, 2148 edges, diameter 1.333). 
%As large-scale unweighted graph, we use Amazon co-purchasing network (334,863 vertices, 925,872 edges, diameter 42)~\cite{yang2015defining}. It is 
\vspace{-1em}
% {To be used for validating the bound on lazy witness approximation. To validate the bound on size we use the }
\subsection{Experimental Setup}\vspace{-.5em}
We implement the experimental workflow in C++. We use Snap library~\cite{leskovec2016snap} for graph processing and $\epsilon$-net computations. We modify the Ripser\Ripser library to compute lazy witness complexes and their persistent intervals.  We use R-TDA package~\cite{rTDA} to compute bottleneck distances. All experiments are run on a machine with an Intel(R) Xeon(R)@2.20GHz CPU and 80 GB memory limit. We set the lazy witness parameter $\nu = 1$ in all computations. We set the maximum value of the filtration parameter to the diameter of the corresponding dataset. We compute persistent intervals at dimension 0 and 1. 

% for impldataset preprocessing, implementing the landmark selection heuristics, constructing the lazy witness filtrations and computing the birth and death of the homology classes. 
% {\color{red}We use matlabs core graph and network algorithm library to compute the centrality scores.} 
 
\begin{figure}[t!]
    \centering
    \includegraphics[width=0.9\textwidth]{efficiencyplots/celegans_final_effic.pdf}
    \caption{Performance of the algorithms on Celegans dataset.}
    \label{fig:effi_cel}
\end{figure}
\begin{figure}[t!]
    \centering
    \includegraphics[width=0.9\textwidth]{efficiencyplots/power_effic.pdf}
    \caption{Performance of the algorithms on Power dataset.}
    \label{fig:effi_pow}
\end{figure}\vspace{-1em}
\subsection{Efficiency and Effectiveness}%\vspace{-1em}
We measure the efficiency of our algorithms in terms of CPU time (in ms) required to select $\epsilon$-net landmarks for a given $\epsilon$, and the overall computation of persistent homology of each graph. The overall total computation time includes the time an algorithm spends constructing $\epsilon$-net and time spent on computing persistent intervals at dimension 0 and 1. 
We measure the effectiveness of the algorithms using the number of landmarks they select by corresponding $\epsilon$-net construction.

Figures~\ref{fig:effi_cel} and~\ref{fig:effi_pow} illustrate the experimental results for the Celegans and the Power dataset respectively. We observe that the number of landmarks selected by all the algorithms decrease as the $\epsilon$-increases. 
The landmark selection time of the Greedy-$\epsilon$-Net increases as the $\epsilon$ increases independent of the dataset.
For other two algorithms, the landmark selection time varies depending on the density of the graph. %As Celegans is a denser graph, 
The landmark computation time of Iterative-$\epsilon$-net and SPTpruning-$\epsilon$-net are almost invariant with $\epsilon$. %For a sparser graph like Power, the landmark selection time decreases rapidly with $\epsilon$.

We observe that Iterative-$\epsilon$-Net takes longer time ($>10$ ms) to select landmarks compared to the SPTpruning-$\epsilon$-Net algorithm but it selects less number of landmarks than SPTpruning-$\epsilon$-Net algorithm. Thus, the overall runtime of lazy witness complex construction using Iterative-$\epsilon$-Net is smaller than that of the SPTpruning-$\epsilon$-Net. The empirical performance analysis instantiates Iterative-$\epsilon$-Net as the practical and efficient choice to construct $\epsilon$-net induced lazy witness complex for graphs.

\begin{figure}[t!]
    \centering\vspace{.2em}
    \includegraphics[width=0.6\textwidth,trim={5cm 7.2cm 5cm 7.2cm}]{valid_figs/celegans_validation.pdf}
    \caption{Validation of the approximation guarantee of the $\epsilon$-net induced lazy witness complexes for Celegans dataset. The bottlneck distance between the partial persistence diagram of the corresponding Vietoris-Rips and lazy witness filtrations is less than $3\log{3}$ in both dimensions 0 and 1.}
    \label{fig:val}
\end{figure}\vspace*{-2.5pt}
% \subsection{Effectiveness expt.}
% We validate the approximation guarante 
% \subsubsection{Size of the $\epsilon$-nets} Figure~\ref{fig:eps_sz}

% \begin{figure}[t!]
% \centering
% \begin{minipage}{.33\textwidth}
%   \centering
%   \includegraphics[width=0.85\textwidth]{ATDA2019/epssize/amazon.pdf}
% \end{minipage}\hfill
% \begin{minipage}{.33\textwidth}
%   \centering
% \includegraphics[width=0.85\textwidth]{ATDA2019/epssize/dblp.pdf}
% \end{minipage}
% \caption{\label{fig:eps_sz}Relation between $\epsilon$ and the number of landmarks generated by the algorithms.}
% \end{figure}

\subsection{Validating the Approximation Guarantee}\vspace*{-1em}
In order to validate the approximation guarantee in Theorem~\ref{thm:approx}, we construct the Vietoris-Rips complex and lazy witness complexes using $\epsilon$-nets for different values of $\epsilon$ and different algorithms. We compare the corresponding complexes by computing bottleneck distances between the persistence diagrams at dimension 0 and 1. We retain only the partial diagram with points in the diagram born after $2\epsilon$ for this purpose. Figure~\ref{fig:val} validates the guarantee on Celegans dataset. We omit the validation on Power dataset for the sake of brevity. 

% \section{Application to Graph Clustering}
% In this section we consider unweighted graphs. But our approach can be generalized to weighted graphs as well. 
% \subsection{$\epsilon$-cover based measures of local Density on graphs}
% A local density measure on an unweighted graph $G = (V,E)$ is a function $f: V \rightarrow \mathbf{R^{+}}$ that captures how clustered or dense the graph is in the neighborhood of its vertices. There many other measures such as degree, various centrality measures that captures local structural properties of a graph. For the purposes of graph clustering we focus on local density measures based on the subgraph induced by the $\epsilon$-neighborhoods of the vertices. 

% One such measure that generalizes the notion of local clustering coefficient is notion of \emph{$\epsilon$-neighbor clustering coefficient}, denoted as $CC_\epsilon$, and is defined for a vertex $v$ as the proportion of edges between the vertices within $v$'s $\epsilon$-neighbourhood divided by the number of edges that could possibly exist between them. For $\epsilon=1$ the definition coincides with the classical local clustering coefficient. Figure ~\ref{fig:cl1} illustrates the value of $CC_\epsilon$ for each vertex. 

% Another measure that generalizes the notion of degree is the size of an $\epsilon$-neighborhood, denoted as $|\mathcal{N}_\epsilon|$, and is defined for a vertex $v$ as the number of vertices in the $\epsilon$-neighborhood of $v$. For $\epsilon=1$ the definition coincides with degree.

% \subsection{Superlevel-set filtration of density functions:} 
% The superlevel-set $V^\alpha = f^{-1}([\alpha,+\infty])$ of a local density function $f$ on the vertices of graph $G = (V,E)$ is a set of vertices whose density is at least $\alpha$. The family of such superlevel-sets has the property that $V^{\alpha} \subseteq V^\beta$ whenever $\beta \leq \alpha$. Persistence of the homology classes of this filtration is different from that of the filtration induced by graph geodesic. Figure~\ref{fig:supset} illustrates the superlevel sets of $CC_\epsilon$ on graphs. As we swipe the parameter $\alpha$ of the filtration from $+1$ down to $0$ connected components are born and merged. The lifespan of each connected component can be represented in the persistent diagram of $CC_\epsilon$.

% %\begin{figure}[t!]
% %	\centering
% %	\begin{minipage}{.24\textwidth}
% %		\centering
% %		 \includegraphics[height=0.25\textheight]{ATDA2019/levelset_g/graph4.pdf}
% %		 \captionof{figure}{\label{fig:graph1} An example}
% %	\end{minipage}\hfill
% %\end{figure}

% \begin{figure}[t!]
% 	\includegraphics[width=0.24\textwidth,trim=2cm 2cm 2cm 2cm]{ATDA2019/levelset_g/graph4.pdf}
% 	%\caption{\label{fig:torus_img} Torus}
% 	\includegraphics[width=0.24\textwidth,trim=2cm 2cm 2cm 2cm]{ATDA2019/levelset_g/graph3.pdf}\hfill
% 	%\caption{\label{fig:ttorus_img} Tangled-torus}
% 	\includegraphics[width=0.24\textwidth,trim=2cm 2cm 2cm 1cm]{ATDA2019/levelset_g/graph2.pdf}\hfill
% 	\includegraphics[width=0.24\textwidth,trim=2cm 2cm 2cm 1cm]{ATDA2019/levelset_g/graph1.pdf}
% 	\centering 
% 	\includegraphics[width=0.5\textwidth]{ATDA2019/levelset_g/pd.pdf}
% 	\caption{\label{fig:supset}(Top row, left to right)  The graph induced by level set $V^{1}$, $V^{0.7}$, $V^{0.67}$ and $V^{0.5}$. (Bottom row) The persistence diagram of the superlevel-set filtration in the top row. The point (0.67,0.5) corresponds to the two components born at 0.67 but merged at 0.5.}
% \end{figure}

% \subsection{Local Density-based graph clustering:}

% {\color{blue}{We adapt ToMATo (Topological Mode Analysis Tool) proposed by Chazal et. al.~\cite{chazal2013tomato} clustering algorithm for point-cloud to graphs. 

% (What Tomato Does) Given a point-cloud $P$, Tomato requires the neighborhood graph $G$ of the point-cloud, and a density estimator $\hat{f}$ of an unknown density function $f:P \rightarrow \mathbf{R}$. ToMATo uses the 0-dimensional persistence diagram of the super level sets $F_\alpha = \hat{f}^{-1}(\alpha,\infty)$ of $\hat{f}$ to determine a provably robust value of density threshold parameter $\tau>0$. Note that, as the level $\alpha$ is decreased from $+\infty$ to $−\infty$ the sets $F_\alpha$ grow, and in this process components and cycles are born and destroyed. \textbf{The birth of a new components is equivalent to the birth of a new cluster and the death of that component is equivalent to its corresponding cluster being merged to another cluster.} 

% After the parameter $\tau$ is chosen, ToMATo performs a mode-seeking (similar to mean-shift algorithm) to compute a collection of trees in the graph where the root of each tree identifies the vertex with the highest $\hat{f}$ value among the neighbors. These collection of trees are the initial clusters. Then it performs a merging step where every cluster(tree) of persistence less than $\tau$ is merged to its parent cluster(tree) in the persistence hierarchy. The output of ToMATo is the collection of trees as clusters whose root has density at least $\tau$. The trees with density less than $\tau$ are discarded as noise. 
%  }}

% (What we do) The neighborhood information of the vertices of a given graph is encoded in the graph itself. However we require a density function on the vertices of the graph that can characterize the local density around the vertices. 
% We propose to use the local density estimate using the landmark. The use the size of the $\delta$-cover of a landmark as local density around that landmark. A special case of this density estimate is the degree of the landmarks.
% Another measure is the ratio of the number of edges in the epsilon-cover and all possible edges that could have been between the vertices in the cover. Both measures require a parameter $\delta$ to be defined. We experiment with both of the local-density estimates.

% We modify ToMaTo to use only landmarks as the root of the tree in the forest. The $\epsilon$-cover of each landmark is the corresponding cluster. The merging of two landmarks effectively merges there associated covers as well. Decision about merging two landmarks uses the same criteria used in ToMaTo. 

% % In our experiment we replace the point-cloud density estimator $\hat{f}$ with \textbf{degree distribution} of the graph.

% \subsection{Experimental Analysis}
% \textbf{Dataset.} LFR Benchmark: We generate three synthetic graphs with Non overlapping ground-truth community structure to measure the quality of the clustering generated. The quality is measured in terms of Normalized mutual information.  

% \textbf{Cluster quality measure.}
% The algorithm generates a partition of the set of vertices where each partition is considered as a cluster. To measure the quality of the clusters generated, given the ground truth from a dataset, many external measures exists, such as the  


% \textbf{Result of the clustering.} TO DO

% % For temporal graphs, ClustNet ~\cite{crawford2018cluenet} and Thesis by Dimitri Lozeve~\cite{} provides algorithms based on persistence homology for temporal graph clustering.

% %\subsection{Application to Graph classification via persistence based Kernels.}
% %Differentiate rangom graphs generated by random graph models via persistence kernel. Works on persistence-based kernel methods~\cite{kwitt2015statistical}~\cite{kusano2016persistence},
% %~\cite{carriere2017sliced}~\cite{zhu2016stochastic}~\cite{le2018persistence}. The difference between traditional graph kernel based methods and persistence-based kernel methods. Recent paper on persistence based graph classification~\cite{JMLR2019}. 
% %
% %\subsection{Application to Graph visualization.}
% %Application of TDA for graph visualization~\cite{hajij2018visual}~\cite{suh2017driving}. 
% %Adapt our $\epsilon$-net induced features for graph visualization.


==> README <==
This package provides a class for typesetting publications of 
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see
Installation section of the User's Guide.

Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.  
		Footnotes rearranged.
                Option natbib is now mostly superfluous: the class 
		makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
		Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
		file is used for all styles.  Better treatment
		of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend;  should be 
		invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29	Documentation changes.  Head height increased from 12pt to 13pt.
		Removed spurious indent at start of abstract.
		Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
	        Added \frenchspacing.
		\department now has an optional hierarchy level.
		Switched to T1 encoding
		Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
		(thanks to Matteo Riondato)
		Table of contents now works
		Marginalia now work in all formats
		New command \additionalaffiliation
		Documentation changes

version 1.32    New DOI formatting.
		Format siggraph is now obsolete, and sigconf
		is used instead.
		New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
		New option `authordraft'
                Documentation updates
		Bug fixes
		We now use Type 1 versions of Libertine fonts even with XeTeX.
		New hook acmart-preload-hook.tex (wizards only!)
		Added new options `obeypunctuation' for \affiliation command
		Added SubmissionID
		Added right line count ruler for two-column formats
		Added workaround for Adobe Acrobat bugs in selection
		Added eid field to the bibliography
		
version 1.34    Deleted DOI from doi numbers
		Changed bibstrip formatting
		The command \terms is now obsolete
		The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.


==> background.tex <==
\section{Topological Data Analysis}\label{sec:tda}%\vspace{-.5em}
Topological data analysis is the study of computational models for efficient and effective computation of topological features, such as persistent homology classes, from different datasets, and representation of the topological features using different topological descriptors, such as persistence barcodes, for further analysis and application~\cite{edelsbrunner2010computational,otter2017roadmap}.
In this section, we represent the computational blocks of topological data analysis in Figure~\ref{fig:pipeline} and further describe each of the blocks.
\begin{figure}[!htbp]
    \centering
    \includegraphics[width=0.4\textwidth]{blocks/TDA_pipeline.pdf}
    \caption{Components of topological data analysis.}
    \label{fig:pipeline}
\end{figure}

Topological data analysis computes the topological features, such as persistent homology classes, by computing the topological objects called \emph{simplicial complex} for a given dataset. A \textbf{simplicial complex} is constructed using simplices. Formally, a \emph{$k$-simplex} is the convex-hull of $(k+1)$ data points. For instance, A 0-simplex $[v_0]$ is a single point, a 1-simplex $[v_0v_1]$ an edge, and a 2-simplex $[v_0v_1v_2]$ a filled triangle. 


\color{red}A \textbf{$k$-homology class} is an equivalent class of such $k$-simplicial complexes that cannot be reduced to a lower dimensional simplicial complex~\cite{edelsbrunner2010computational}.


In order to compute the $k$-homology classes, a practitioner does not have direct access to the underlying space of the point cloud and it is combinatorially hard to compute the exact simplicial representation of \v Cech complex~\cite{zomorodian2010fast}.
Thus, different approximations of the exact simplicial representation are proposed: \emph{Vietoris-Rips} complex~\cite{hausmann1995vietoris} and \emph{lazy witness} complex~\cite{de2004topological}.

The \textbf{Vietoris-Rips complex} $R_\alpha(D)$, for a given dataset $D$ and real number $\alpha > 0$, is an abstract simplicial complex representation consisting of such $k$-simplices, where any two points $v_i, v_j$ in any of these $k$-simplices are at distance at most $\alpha$. Vietoris-Rips complex is the best possible ($\sqrt{2}$-)approximation of the \v Cech complex, computable with present computational resources, and is extensively used in topological data analysis literature~\cite{otter2017roadmap}. Thus, we use the Vietoris-Rips complex as the baseline representation in this paper.
In the worst case, the number of simplices in the Vietoris-Rips complex grows exponentially with the number of data points~\cite{otter2017roadmap,zomorodian2010fast}. 
Lazy witness complex~\cite{de2004topological} approximates the Vietoris-Rips complex by constructing the simplicial complexes over a subset of data points $L$, referred to as the landmarks. 
% Though this approximation leads to loss of topological features, lazy witness complex captures a portion of the topological features of the underlying space depending on the choice of landmarks. 
% \vspace*{-1em}
% \begin{definition}[Lazy Witness Complex~\cite{de2004topological}]
Formally, given a positive integer $\nu$ and real number $\alpha>0$, the \textbf{lazy witness complex} $LW_\alpha(D,L,\nu)$ of a dataset $D$ is a simplicial complex over a landmark set $L$ where for any two points $v_i,v_j$ of a $k$-simplex $[v_0 v_1\cdots v_k]$, there is a point $w$ whose $(d^\nu(w) + \alpha)$-neighbourhood\footnote{$d^\nu(w)$ is the  geodesic distance from point $w \in V$ to its $\nu$-th nearest point in $L$.} contains $v_i, v_j$.
%\end{definition}\vspace{-1em}
In the worst case, the size of the lazy witness complexes grows exponentially with the number of landmarks. Less number of landmarks facilitates computational acceleration while produces a bad approximation of Vietoris-Rips with loss of topological features. Thus, the trade-off between the approximation of topological features and available computational resources dictates the choice of landmarks. We provide a quantification on such loss of topological features  which was absent in the literature.

%For a given filtration parameter $\alpha$, the Rips and lazy witness complex provide corresponding approximate simplicial complex representations.
As the value of filtration parameter $\alpha$ increases, new simplices arrive and the topological features, i.e. the homology classes, start to appear. Some of the homology classes merge with the existing classes in a subsequent simplicial complex, and some of them persist indefinitely~\cite{edelsbrunner2010computational}.
In order to capture the evolution of topological structure with scale, topological data analysis techniques construct a sequence of simplicial complex representations, called a \emph{filtration}~\cite{edelsbrunner2010computational}, for an increasing sequence of $\alpha$'s. 
In a given filtration, the persistence interval of a homology class is denoted by $[\alpha_{b},\alpha_{d})$, where $\alpha_{b}$ and $\alpha_{d}$ are the filtration values of its appearance and merging respectively. The persistence interval of an indefinitely persisting homology class is denoted as $[\alpha_{b},\infty)$.
Topological descriptors, such as barcodes~\cite{collins2004barcode}, persistence diagram~\cite{edelsbrunner2010computational}, and persistence landscapes~\cite{bubenik2015statistical}, represent persistence intervals in order to draw qualitative and quantitative inference about the topological features. Distance measures between persistent diagrams such as the q-Wasserstein and Bottleneck distance~\cite{edelsbrunner2010computational} are often used to draw quantitative inference.
